Gromov boundary of the Grand Arc graph

We describe a dense subset of the Gromov boundary of the grand arc graph of an infinite-type surface as a space of geodesic laminations, analogous to Klarreich's description of the Gromov boundary of the curve complex. After showing that the grand arc graph satisfies a bounded geodesic image theorem, we also prove that the boundary is not compact.

==> Future-Ideas.tex <==
This is a place to write some ideas, conjectures, and longer-term ideas that put the work into context.

Aug. 21: Lemma 7.2.1 of https://arxiv.org/pdf/1806.10272.pdf essentially says that if we add "limit sets of HF lines," then in the case of a partial pseudo-Anosov f, the connected components of HF rays defining the the attracting point on the boundary corresponding to f is a cone. -ABN

Aug. 21: Attracting points of partial pseudo-Anosovs may indeed dense in the boundary. Consider a HF line, look at its limset, and view that as a lamination. Note that this lamination has no leaves converging to punctures. Saric says that there's a train-track that carries this lamination. Now, take a finite subset of this train-track, and choose it carefully so that it is chain-recurrent. Then take a partial pseudo-Anosov that has an attracting lamination carried by this train-track. Since both the HF line and the attracting lamination are carried by the same train-track, the attracting lamination should be Hausdorff close  to the HF line. It seems like taking larger and larger sub-train-tracks would then give a CHCCS sequence of finite-type laminations that come from partial pseudo-Anosovs that then converge to the HF line. -ABN

Aug. 21: If the above is true, then it is a very strong restriction on infinite-type loxodromic mapping classes. I'd be really interested to know if this means that all mapping classes that act loxodromically on the grand arc graph lie in the closure of the compactly supported mapping classes. - ABN

Aug 29: We need some notion of minimality. Basically there are two notions "Hausdorff distance" - in the graph, and on the surface. CHCCS talks about convergence on the surface. Our bicorn paths are constructed so that we are disjoint from a grand line for longer and longer regions along the grand line. But unless the grand line is somewhat "minimal", this disjointness may not translate to "being Hausdorff close on the surface". 

==> Modules/Bavard-Walker.tex <==
\section{The once-punctured Cantor tree}\label{sec:BW_stuff}

In this section, we restrict to the case that $\Sigma$ is the once-punctured Cantor tree. There are two elements in the grand splitting for $\Sigma$, one corresponding to the isolated puncture, which we denote by $\infty$, and the other corresponding to a Cantor set of ends, which we denote by $K$. The \textit{ray graph} of $\Sigma$ was defined by Calegari as the graph whose vertices correspond to isotopy classes of proper arcs between  $\infty$ and a point in $K$ and whose edges corresond to disjointness.  Bavard showed that this is an infinite-diameter hyperbolic graph \cite{Bav}, and it is exactly equal to $\mathcal{G}\left(\Sigma\right)$. 

The ray graph is a special case of the more general class of \textit{relative arc graphs}, defined by Aramayona, Fossas, and Parlier for surfaces with at least one isolated puncture \cite{AFP}, but for surfaces other than the once-punctured Cantor tree, relative arc graphs do not coincide with the grand arc graph.

Bavard and Walker \cite{B-W} show that the Gromov boundary of the ray graph is homeomorphic to the space $\mc E$ of connected components of \textit{high-filling rays}; see \cite[Definition 2.7.1]{B-W} for a precise definition.  A \textit{ray} on $\Sigma$ is a simple geodesic converging to $\infty$. The topology on $\mc{E}$ is a quotient of the topology on $\mc{H}$, the space of high-filling rays on $\Sigma$ considered as a subspace of $\Gamma(\Sigma)$ with the topology of geodesic convergence.


In this section, we explore the relationship between $\mathcal{GEL}\left(\Sigma\right)$ and the space $\mathcal{E}$. In particular, we will show in Proposition~\ref{prop:cliques_equal_GEL} that $\mathcal{GEL}$ is homeomorphic to a subspace $\mc E_{min}$ of $\mc E$. 


To describe the subset $\mc E_{min}$, we first define the \textit{limit set} of a ray. %The connection between a ray and a geodesic lamination comes from the \textit{limit set} of the ray.
For any geodesic $\gamma$ on $\Sigma$, let $\mathrm{cl}(\gamma)$ be the closure of $\gamma$ in $\Gamma\left(\Sigma\right)$.  The \textit{limit set} $\lim(\gamma)$ of $\gamma$ is the collection of geodesics $\mathrm{cl}(\gamma)\backslash\gamma$. 
\begin{lem}
If $l$ is a ray on $\Sigma$, then $\mathrm{cl}(l)$ and $\lim(l)$ are geodesic laminations.
\end{lem}

\begin{proof}
By definition, $\mathrm{cl}(l)$ is closed. Since $l$ converges to the isolated puncture $\infty$, there is an annular neighbourhood of $\infty$ that $l$ intersects in a single radial arc; see, for example, \cite[Lemma 2.4.2]{B-W}. Thus, $l\subseteq\mathrm{cl}(l)$ is an isolated geodesic, and so $\lim\left(l\right)$ is also closed. Moreover, two geodesics in $\mathrm{cl}(l)$ cannot transversely intersect, as $l$ geodesically converges to both and is simple. It follows that both $\mathrm{cl}(l)$ and $\lim(l)$ are geodesic laminations.
\end{proof}


It will be useful to recall some terminology from \cite{B-W}.  A \textit{loop} is a ray that converges to $\infty$ in both directions.  A \textit{short ray} (or a \textit{0-filling ray}) is a ray between $\infty$ and a point in $K$; isotopy classes of short rays form the vertex set of the ray graph.  A \textit{long ray} is a ray that converges to $\infty$ in one direction and does not converge to either $\infty$ or a point of $K$ in the other.  A ray is \textit{filling} if it intersects every loop and short ray. A ray is \textit{$k$-filling} for some $k\geq 1$ if it is not $(k-1)$-filling, but is disjoint from a $(k-1)$-filling ray. A ray is \textit{high-filling} if it is not $k$-filling for any $k\geq 0$.

A clique $C$ of high filling rays has a well-defined limit set:  if $l,m\in C$, then $\lim(l)=\lim(m)$ by \cite[Lemma 6.3]{CR}.  Define $\lim(C)$ to be $\lim(l)$ for some (equivalently, any) $l\in C$.  Note that high-filling rays are, in particular, filling.  We define $\mc E_{\textrm{min}}\subseteq \mc E$ to be the subspace of $\mc E$ consisting of cliques $C$ of high-filling rays such that $\lim(C)$ is a minimal geodesic lamination, that is, such that $\lim(C)\in \mc{GEL}(\Sigma)$.  

%Let $C$ be a clique of high-filling rays, and let $l\in C$. By \cite[Lemma 6.3]{CR}, we see that for any other $m\in C$, $\lim(m)\subset\lim(l)$. Consequently, we have that $\lim(l)=\lim(m)$ for any $l,m\in C$. We can thus define a lamination $\lim(C)$ as $\lim(l)$ for any $l\in C$. Since each $l\in C$ is arc-filling, $\lim(C)$ is witness-filling. We conjecture that $\lim(C)$ is also minimal, so that $\lim (C)\in \mc{GEL}(\Sigma)$.


\begin{prop}\label{prop:cliques_equal_GEL}
The map
\[
f\colon \mathcal{E}_{\min}\to\mathcal{GEL}\left(\Sigma\right)
\]
given by \[f(C)=\lim(C)\] is a homeomorphism.
\end{prop}



%We conjecture the answer to be ``yes''.


%Bavard and Walker in \cite[Section 7.2]{B-W_2} previously established this for finite-type surfaces with an isolated puncture, where they prove that rays asymptotic to the attracting or repelling laminations of a pseudo-Anosov homeomorphism correspond to cliques of high-filling rays. We claim that this works more generally. 


% But for now, define $\mathcal{E}_{\mathrm{min}}$ to be the subspace of $\mc{E}$ consisting of cliques $C$ of high-filling rays such that $\lim(C)$ is a minimal geodesic lamination. That is to say, $\lim(C)\in\mathcal{GEL}\left(\Sigma\right)$. 



 To prove Proposition \ref{prop:cliques_equal_GEL}, we define a map $g$ which we shall prove to be the inverse of $f$, and show that both $f$ and $g$ are continuous.

\begin{lem}\label{lem:map_GEL_to_E}
Let $L\in\mathcal{GEL}\left(\Sigma\right)$.  The set
\[
C_{L}=\left\{ \tau\mid\tau\text{ is a long ray disjoint from \ensuremath{L} and asymptotic to }L\right\}
\]
is a clique of high-filling rays in $\mc E_{\textrm{min}}$.
\end{lem}

\begin{proof}
Let $L\in\mathcal{GEL}\left(\Sigma\right)$. We first show that $C_{L}$ is non-empty.  To see this, notice that as $L$ stays disjoint from an annular neighbourhood of the isolated puncture $p$, we can choose a radial arc converging to the isolated puncture in this annular neighbourhood.  Connect this arc with a shortest path to a boundary leaf of $L$ and then follow along this leaf in either direction to construct a long ray in $C_{L}$. 

Fix any $\tau\in C_L$.  Since $L$ is minimal, we have  $\lim\left(\tau\right)=L$ by definition. As $L$ is witness-filling,  $\tau$ must be filling, and if $\tau$ were $2$-filling, then \cite[Proposition 6.4]{CR} would imply that $L$ is not minimal. Thus, $\tau$ is high-filling. If $\tau,\tau'\in C_{L}$ with $\tau\cap\tau'\neq\emptyset$, then we can construct a loop in the unicorn path between $\tau$ and $\tau'$ that is disjoint from $L$. However, this would contradict that $L$ is witness-filling: if $\supp(L)$ is a witness, then $L$ must intersect every arc, and hence every loop by  \cite[Lemma 2.7.2]{B-W}. 

Thus, $C_{L}$ is a clique of high-filling rays; in fact, this is the full clique by \cite[Lemma 6.3]{CR}. Moreover, as each $\tau\in C_L$ is asymptotic to $L$, which is minimal, we much have that $\lim(C)=\lim(\tau)\subseteq L$ is minimal.  Thus $C_L\in \mc{E}_{\min}$. %Thus, setting $g\left(L\right)=C_{L}$ gives us a well-defined map $g:\mathcal{GEL}(\Sigma)\to\mathcal{E}_{\min}$.
\end{proof}

By Lemma~\ref{lem:map_GEL_to_E}, there is a well-defined map
\[
g\colon \mathcal{GEL}\left(\Sigma\right)\to\mathcal{E}_{\min}
\]
 by 
 \[
 g(L)=C_{L}.
 \]

\begin{lem}\label{lem:BW_bijections}
The maps $f$ and $g$ are both bijective, and are inverses of each other.
\end{lem}

\begin{proof}
We first show that $f\circ g=\mathrm{id}_{\mathcal{GEL}\left(\Sigma\right)}$. Let $L\in\mathcal{GEL}\left(\Sigma\right)$, let $g(L)=C_{L}$. By definition, since any $\tau\in C_{L}$ is asymptotic to $L$, we have $L\subset\lim\left(\tau\right)=\lim\left(C_{L}\right)$. Since $C_L\in \mc{E}_{\min}$, $\lim\left(C_{L}\right)$ is minimal, so in fact $L=\lim\left(C_{L}\right)=f(C_L)=f\circ g(L)$.

For the other composition, let $C\in\mathcal{E}_{\min}$, and let $L=\lim(C)=f(C)$. For any $\tau\in C$, we have $\lim\left(\tau\right)=L$. In particular, $\tau$ is a long ray that is disjoint from $L$ and asymptotic to $L$, so $\tau\in C_{L}$. Conversely, if $\gamma\in C_{L}$ is a long ray, then $L=\lim\left(\gamma\right)$. As in the proof of Lemma \ref{lem:map_GEL_to_E}, if $\gamma$ intersects some $\gamma'\in C$ transversely, then we can construct a loop in the unicorn path between $\gamma$ and $\gamma'$ which is disjoint from $L$, contradicting that $L\in\mathcal{GEL}\left(\Sigma\right)$. Thus, $\gamma$ is disjoint from any $\gamma'\in C$, so we must have $\gamma\in C$. Thus, $C=C_{L}=g(L)=g\circ f(C)$.
\end{proof}

%So we have a bijective map $f:\mathcal{E}_{\min}\to\mathcal{GEL}\left(\Sigma\right)$. To conclude the proof of Proposition \ref{prop:cliques_equal_GEL} would like to now show that $f$ and $g$ are continuous. 
To prove Proposition~\ref{prop:cliques_equal_GEL}, it remains to show that $f$ and $g$ are continuous.  We begin with a preliminarly lemma that relates the convergence of a sequence of geodesics to convergence of their closures. 


\begin{lem}
\label{lem:limit_of_limits}Suppose $\left(\gamma_{n}\right)_{n\in\mathbb{N}}$ is a sequence of geodesics on $\Sigma$  that geodesically converges to a geodesic $\gamma$.  For any $\gamma_{n}'\in\mathrm{cl}\left(\gamma_{n}\right)$ and $\gamma'\in\mathrm{cl}\left(\gamma\right)$, we have that $\gamma_{n}'\xrightarrow{\mathrm{geod}}\gamma'$. In particular, $\mathrm{cl}\left(\gamma_{n}\right)\xrightarrow{CC}\mathrm{cl}\left(\gamma\right)$ and $\lim(\gamma_n)\xrightarrow[]{CC}\lim(\gamma)$.
\end{lem}

\begin{proof}
\end{proof}
Since $\gamma_{n}\xrightarrow{\mathrm{geod}}\gamma$, for any lift $\tilde{\gamma}$ of $\gamma$ to the universal cover $\mathbb{H}^{2}$ of $\Sigma$, there is a corresponding sequence of lifts $\tilde{\gamma}_{n}$ of $\gamma_{n}$ which converges to $\tilde{\gamma}$ in $\Gamma\left(\mathbb{H}^{2}\right)$. For each $n$, since $\gamma'_{n}\in\mathrm{cl}\left(\gamma_{n}\right)$, there is a lift $\tilde{\gamma}_{n}'$ of $\gamma_{n}'$ arbitrarily close to $\tilde{\gamma}_{n}$ in $\Gamma\left(\mathbb{H}^{2}\right)$. Similarly, since $\gamma'\in\mathrm{cl}\left(\gamma\right)$, there is a lift $\tilde{\gamma}'$ of $\gamma'$ arbitrarily close to $\tilde{\gamma}$. Consequently, $\left(\tilde{\gamma}_{n}'\right)_{n\in\mathbb{N}}$ converges to $\tilde{\gamma}'$ in $\Gamma\left(\mathbb{H}^{2}\right)$, and so $\gamma_{n}'\xrightarrow{\mathrm{geod}}\gamma'$. 
%




\begin{cor}\label{lem:BW_f_cont}
The map $f\colon \mathcal{E}_{\min}\to\mathcal{GEL}\left(\Sigma\right)$ is continuous.
\end{cor}

\begin{proof}
It was shown in \cite{B-W} that $\mc E$, and hence $\mathcal{E}_{\min}$, is first-countable, so it suffices to show that $f$ is sequentially continuous. 

Let $\left(C_{n}\right)_{n\in\mathbb{N}}\subset\mathcal{E}_{\min}$ be a sequence such that $C_{n}\to C$ for some $C\in\mathcal{E}_{\min}$.  As $\mc E_{\textrm{min}}\subseteq \mc E$ has the subspace topology, it follows that for every $\tau\in C$, there exists $\tau_{n}\in C_{n}$ such that $\tau_{n}\xrightarrow{\mathrm{geod}}\tau$. By Lemma \ref{lem:limit_of_limits}, $\lim\left(\tau_{n}\right)\xrightarrow{CC}\lim\left(\tau\right)$, and so $f\left(C_{n}\right)\to f\left(C\right)$, as desired.
\end{proof}
%

A key tool in the proof that $g$ is continuous is the \textit{conical cover} of $\Sigma$.  This cover is defined precisely in \cite[Section~2.2]{B-W}, but the key points we will use here is that it contains a preferred lift $\tilde\infty$ of $\infty$, and the boundary of the conical cover is a homeomorphic to $\mathbb S^1$.  When we lift a ray $r$ in $\Sigma$ converging to $\infty$ to a ray $\tilde r$ in the conical cover, we always assume that it converges to the preferred lift $\tilde \infty$.
\begin{lem}\label{lem:BW_g_cont}
The map $g\colon \mathcal{GEL}\left(\Sigma\right)\to\mathcal{E}_{\min}$ continuous. 
\end{lem}

\begin{proof}
By Corollary \ref{cor:seq_continuity}, it suffices to show that $g$ is sequentially continuous. Suppose $\left(L_{n}\right)_{n\in\mathbb{N}}\subset\mathcal{GEL}\left(\Sigma\right)$ is a sequence satisfying $L_{n}\xrightarrow{CC}L$ for some $L\in\mathcal{GEL}\left(\Sigma\right)$. Let $r\in g\left(L\right)$ be a high-filling ray. We will construct a sequence of high-filling rays $r_{n}\in g\left(L_{n}\right)$ such that $r_{n}\xrightarrow{\mathrm{geod}}r$. 

Let $\tilde{r}$ be a lift of $r$ to the conical cover of $\Sigma$. Since $r$ is asymptotic to $L$, there is a parametrized leaf $l\in L$ such that  $\lim_{t\to\infty}d_{\Sigma}\left(l(t),r(t)\right)=0$. Thus, there exists a lift $\tilde{l}$ of $l$ such that one of the endpoints, say $\tilde l (\infty)$, of $\tilde l$ on the boundary of the conical cover is the same as the endpoint $\tilde{r}(\infty)$ of $\tilde r$. As $L_{n}\xrightarrow{CC}L$, there is a sequence of leaves $l_{n}\in L_{n}$ such that $l_{n}\xrightarrow{\mathrm{geod}}l$, and by Lemma \ref{lem:convg_as_geod}, there exist lifts $\tilde{l}_{n}$ of $l_{n}$ which converge to $\tilde{l}$. In particular, the sequence of endpoints $(\tilde{l}_{n}(\infty))_{n\in \mathbb N}$ on the boundary of the conical cover converges to $\tilde{r}(\infty)$. Define geodesics $\tilde{r}_{n}$ in the conical cover by joining $\tilde{\infty}$ to $\tilde{l}_{n}(\infty)$, and let $r_{n}$ denote the projection of $\tilde{r}_{n}$ to $\Sigma$. Then each $r_{n}$ is a long rays on $\Sigma$ asymptotic to $l_{n}$. As in the proof of Lemma~\ref{lem:map_GEL_to_E}, it follows that each $r_{n}$ is high-filling. 
\end{proof}

\begin{proof}[Proof of Proposition \ref{prop:cliques_equal_GEL}]
    This follows from Lemma \ref{lem:BW_bijections}, Corollary \ref{lem:BW_f_cont} and Lemma \ref{lem:BW_g_cont}.
\end{proof}

Proposition~\ref{prop:cliques_equal_GEL} does not show that the full boundary of the ray graph is $\mc{GEL}(\Sigma)$, because $\mc E_{\textrm{min}}$ may be a proper subset of $\mc E$.  However, it is possible that these sets actually coincide:
\begin{question}
Is the limit set $\lim(C)$ of any clique $C$ of high-filling rays a minimal lamination?  That is, is $\mc E=\mc E_{\textrm{min}}$?
\end{question}


The map $F\colon \mc{GEL}(\Sigma)\to\partial\mc{G}(\Sigma)$ defined in Section \ref{sec:GEL_boundary} is only defined for surfaces $\Sigma$ with $|\mc{S}(\Sigma)|\geq 3$, which does not include the once-punctured Cantor tree. However, it is likely that the arguments in this paper can be modified to include this case. We leave this discussion for a future project.

%If Corollary~\ref{cor:unicorn_hausdorff_dist} holds for the once-punctured Cantor tree, the  arguments of Sections \ref{sec:bicorns_with_generic_geod} and \ref{sec:GEL_boundary} would carry over, and the map $F$ would be well-defined on $\mc{GEL}(\Sigma)$.

%Bavard and Walker defined a homeomorphism $\varphi\colon \mathcal{E}\to\partial\mathcal{G}\left(\Sigma\right)$ by $\phi(C)=\left[P\left(a,l\right)\right]$, where $a$ is a loop based at $p$, $l\in C$ is a high-filling ray, and $P\left(a,l\right)$ is the unicorn path between $a$ and $l$ \cite{B-W}. The map $F\colon \mc{GEL}(\Sigma)\to\partial\mc{G}(\Sigma)$ defined in Section \ref{sec:GEL_boundary} is currently only defined for surfaces $\Sigma$ with $|\mc{S}(\Sigma)|\geq 3$, since we prove that finite bicorn sets are unparametrised quasi-geodesics (i.e. Corollary \ref{cor:unicorn_hausdorff_dist}) only in this setting. We conjecture that similar results should also be true for the once-punctured Cantor tree.

%\begin{question}
   % Let $a,b$ be short rays on the once-punctured Cantor tree, and let $\mc{B}(a,b)$ denote the set of bicorn arcs between $a$ and $b$. Then is (a neighbourhood of) $\mc{B}(a,b)$ a uniform quasi-geodesic set?
%\end{question}

%Note that if the answer to the question above is ``yes", then the arguments of Sections \ref{sec:bicorns_with_generic_geod} and \ref{sec:GEL_boundary} carry over, and the map $F$ (via ending bicorn sequences) is well-defined on $\mc{GEL}(\Sigma)$.

%\begin{question}
   % Is there a version of the bounded geodesic image theorem (similar to Theorem \ref{thm:BGI}) true for the ray graph (or the short-ray-and-loop graph)?
%\end{question}

%If the answer to this question is ``yes", then we would expect $F(\mc{GEL}_{\mathrm{cpct}}(\Sigma))$ to be dense in $\partial \mc{R}'$.

%While we leave these questions for future consideration, we note that the map $F$ (if it were defined) would agree with the map $\varphi$. 


%\begin{lem}
%Let $\Sigma$ denote the once-punctured Cantor tree, let $L\in\mathcal{GEL}\left(\Sigma\right)$. Let $l$ be a high-filling ray asymptotic to $L$, and let $m$ be a leaf of $L$. Let $a$ be a loop (based at $p$), and $a'$ be a short ray disjoint from $a$. Then as subsets of the short-ray-and-loop graph of $\Sigma$, we have $\mathcal{P}\left(a,l\right)\subset N_{K}\left(\mathcal{B}\left(a',m\right)\right)$ for some fixed $K>0$.
%\end{lem}

%\begin{proof}
%First note that the choice of $a$ or $l$ only shifts $\mc{P}(a,l)$ by finite Hausdorff distance (as proved in \cite{B-W}), and the choice of $a'$ or $m$ shifts $\mc{B}(a',m)$ by finite Hausdorff distance (by analogues of Lemma \ref{lem:bicorn_changing_first_arc} and \ref{lem:bicorns_with_lamination}). So we assume $m$ is the boundary leaf of $L$ that $l$ asymptotically approaches. We also assume that $a'$ at least $1$-begins-like $l$, so that any intersection of $l$ with $a'$ corresponds to an intersection with $a$ and $m$. 

%Let $u\in\mathcal{P}\left(a,l\right)$ be a unicorn loop. Then $a'\cap u$ is finite; moreover, since $a\cap a'=\emptyset$, all points of $a'\cap u$ are along the $l$-part of $u$. Let $P$ and $Q$ denote the first and the last points of $a'\cap u$ along $a'$. Then the bicorn arc $b=\left(\dots P\right)_{a'}\cup\left(PQ\right)_{l}\cup\left(Q\dots\right)_{a'}$ is simple, and intersects $u$ in at most one point. Moreover, we can find corresponding points of intersection $P',Q'$ of $a'\cap m$, to get a bicorn arc $b'=\left(\dots P'\right)_{a'}\cup\left(P'Q'\right)_{m}\cup\left(Q'\dots\right)_{a'}$ (which is homotopic to $b$) in $\mathcal{B}\left(a',m\right)$. Thus, $u\in N_{2}\left(\mathcal{B}\left(a',m\right)\right)$. 
%\end{proof}

%Thus, if the map $F$ were defined via ending bicorn sequences as in Section \ref{sec:GEL_boundary}, both $\mc{P}(a,l)$ and $\mc{B}(a',m)$ would give points on the Gromov boundary, which would have to be the same point by the above lemma. Thus, we would have a commuting diagram 

%\[
%\xymatrix{\mathcal{GEL}\left(\Sigma\right)\ar^{F}[r]\ar@/^/^{g}[d] & \partial\mathcal{\mathcal{R}}'\\
%\mathcal{E}_{\mathrm{min}}\ar@/^/^{f}[u]\ar_{\varphi}[ur]
%}
%\]

%Understanding the space of minimal witness-filling laminations on $\Sigma$, which is a very concrete space associated to the geometry of $\Sigma$, may help us understand $\mathcal{E}$ better. For example, consider the subspace $g\left(\mathcal{GEL}_{\mathrm{cpct}}\right)\subset\mathcal{E}$. Proving that $F\left(\mathcal{GEL}_{\mathrm{cpct}}\left(\Sigma\right)\right)$ is dense in $\partial\mathcal{G}\left(\Sigma\right)$ translates to proving that $\mathcal{E}_{\mathrm{cpct}}$ (cliques of high-filling rays supported in a finite-type subsurface of $\Sigma$) is dense in $\mathcal{E}$. In particular, the collection of finite cliques of high-filling rays would be dense in $\mathcal{E}$.







==> Modules/Distances_with_laminations.tex <==
\section{Distances with laminations}

In this section, we define a notion of \textit{completed grand arc graph}, similar to the completed ray graph in \cite{B-W}. 
\begin{defn}
Let $\Lambda_{\mathcal{G}}\left(\Sigma\right)\subset\Lambda\left(\Sigma\right)$ be the subspace consisting of connected laminations that intersect every witness of $\mathcal{G}\left(\Sigma\right)$ essentially. 
\end{defn}

\begin{rem}
Note that a single simple closed curve is in $\Lambda\left(\Sigma\right)$ but not in $\Lambda_{\mathcal{G}}\left(\Sigma\right)$. If $\Sigma$ has at least four elements in the grand splitting (so that the smallest witness is a sphere with $n\geq4$ holes), then a pants decomposition of $\Sigma$ intersects every witness of $\mathcal{G}\left(\Sigma\right)$ essentially, but is not in $\Lambda_{\mathcal{G}}\left(\Sigma\right)$ since it isn't connected. If $Y\subset\Sigma$ is a partial witness (as defined in \_\_), then any lamination filling $Y$ is in $\Lambda_{\mathcal{G}}\left(\Sigma\right)$. Finally, any lamination filling a witness is also in $\Lambda_{\mathcal{G}}\left(\Sigma\right)$. 
\end{rem}

\begin{lem}
\label{lem:grand_arcs_wf_lams}A proper arc $\alpha\subset\Sigma$ (when thought of as a lamination with a single leaf) is in $\Lambda_{\mathcal{G}}\left(\Sigma\right)$ if and only if $\alpha\in\mathcal{G}\left(\Sigma\right)$. 
\end{lem}

\begin{proof}
If an end of $\alpha$ is not maximal, then we can find an open neighbourhood of some maximal end (possibly the other end of $\alpha$) which contains both the ends of $\alpha$. Consequently, $\alpha$ is contained in the complement of a witness. 
\end{proof}
%
\begin{lem}
\label{lem:convg_to_wf_lams}Let $\left(x_{n}\right)_{n\in\mathbb{N}}\subset\mathcal{G}\left(\Sigma\right)$ such that $x_{n}\to L$ in the geometric topology, for some $L\in\Lambda\left(\Sigma\right)$. Then $L\in\Lambda_{\mathcal{G}}\left(\Sigma\right)$.
\end{lem}

\begin{proof}
First, each $x_{n}$ is a connected lamination, so $L$ must be connected. Now, since each $x_{n}$ is a grand arc, it has non-trivial intersection with each witness $W\subset\Sigma$. Thus, up to choosing a subsequence, $x_{n}\cap W$ (as laminations in $W$) converge to some lamination $L_{W}\subset W$. By geometric topology, $L_{W}\subset L\cap W$, so $L$ intersects $W$ essentially. 
\end{proof}
\begin{defn}
We define \textit{the completed grand arc graph} $\overline{\mathcal{G}}\left(\Sigma\right)$ as follows: vertices of $\overline{\mathcal{G}}\left(\Sigma\right)$ correspond to elements of $\Lambda_{\mathcal{G}}\left(\Sigma\right)$, and we define an edge between $L_{1},L_{2}\in\Lambda_{\mathcal{G}}\left(\Sigma\right)=\overline{\mathcal{G}}(\Sigma)^{(0)}$ if $L_{1}\pitchfork L_{2}=\emptyset$. 
\end{defn}

In this section, we shall prove the following: 
\begin{thm}
\label{thm:completed_graph_qi}There exists a unique connected component of $\overline{\mathcal{G}}\left(\Sigma\right)$ (denoted $\overline{\mathcal{G}}_{0}\left(\Sigma\right)$), consisting of grand arcs. This component is quasi-isometric to $\mathcal{G}\left(\Sigma\right)$. The other components of $\overline{\mathcal{G}}\left(\Sigma\right)$ correspond to elements of $\mathcal{GEL}\left(\Sigma\right)$. 
\end{thm}

The statement (and the proof which follows) of this theorem are similar to Theorem 2.8.1 of \cite{B-W}. Before we get to proving this, we need to make some additional observations about laminations in $\overline{\mathcal{G}}_{0}\left(\Sigma\right)$. 
\begin{defn}
Let $L\in\overline{\mathcal{G}}\left(\Sigma\right)$. We say that $L$ is:
\begin{enumerate}
\item \textit{0-filling} - if $L$ is a grand arc.
\item \textit{$k$-filling (for some $k>0$)} - if $L$ is not $\left(k-1\right)$-filling, but is distance at most $k$ in $\overline{\mathcal{G}}\left(\Sigma\right)$ from some grand arc. 
\item \textit{high-filling} - if $L\in\overline{\mathcal{G}}\left(\Sigma\right)\backslash\overline{\mathcal{G}}_{0}\left(\Sigma\right)$; equivalently, there is no finite path in $\overline{\mathcal{G}}\left(\Sigma\right)$ from $L$ to a grand arc.
\end{enumerate}
\end{defn}

Similar to Lemma 2.7.6 from \cite{B-W}, we shall prove that there are no $k$-filling laminations for $k>2$. To do this, we shall analyze their supports. Note that for any lamination $L$, we define its support $\mathrm{supp}(L)$ as the subsurface containing $\overline{N_{\epsilon}(L)}$ for some $\epsilon>0$ small. \textcolor{red}{Careful here.}
\begin{lem}[0-filling laminations] \label{lem:0-filling}
A grand lamination $L$ is $0$-filling if and only if $\mathrm{supp}(L)$ is an infinite strip intersecting every witness essentially (or equivalently, $L$ is a single arc in $\Lambda_{\mathcal{G}}$). 

\end{lem}

\begin{proof}
First, if $L$ is $0$-filling (i.e. a grand arc), then we can choose some $\epsilon>0$ small such that $\overline{N_{\epsilon}}(L)$ is an embedded infinite rectangular strip. Conversely, if $\mathrm{supp}(L)$ is homeomorphic to such an infinite strip $\mathbb{R}\times\left[-\epsilon,\epsilon\right]$, then its core $\mathbb{R}\times\left\{ 0\right\} $ is an arc in $\Sigma$. This arc is grand by Lemma \ref{lem:grand_arcs_wf_lams}, since we assume that this strip intersects every witness essentially. 
\end{proof}

\begin{lem}[1-filling laminations] \label{lem:1-filling}
A grand lamination $L$ is $1$-filling if and only if $\mathrm{supp}(L)$ is a partial witness which is not an infinite rectangular strip.
\end{lem}
\begin{proof}
A grand lamination $L$ is 1-filling if and only if $L$ intersects every witness, is disjoint from some grand arc, and is not itself a grand arc. This means that $\mathrm{supp}(L)$ intersects every witness, is not itself a witness (hence is a partial witness), and is not an infinite rectangular strip (by Lemma \ref{lem:0-filling}). 
\end{proof}

\begin{lem}[2-filling laminations]
\label{lem:2-filling laminations} Suppose if $\Sigma$ has at least $4$ elements in the grand splitting. Then a grand lamination $L_{2}$ is 2-filling if and only if $\mathrm{supp}(L_{2})$ is a witness and there is a sublamination $L'\subset L_{2}$ which is 1-filling. 

If the grand splitting for $\Sigma$ has exactly $3$ elements, then $L_{2}$ is 2-filling if and only if $\mathrm{supp}\left(L_{2}\right)$ is a witness and either there is a sublamination $L'\subset L_{2}$ which is 1-filling, or $L_{2}$ contains a sublamination that is the union of two connected components $C_{1}$ and $C_{2}$ disjoint from a common witness, and an isolated leaf asymptotic to them both. 
\end{lem}

\begin{rem}
This is similar to Proposition 6.4 in \cite{CR}.
\end{rem}

\begin{proof}
For the $\impliedby$ direction, if there exists a 1-filling sublamination $L'\subset L_{2}$, then in particular $L'\pitchfork L_{2}=\phi$ showing that $L_{2}$ is at most 2-filling. Then since $\mathrm{supp}\left(L_{2}\right)$ is a witness, Lemma \ref{lem:1-filling} implies that $L_{2}$ is indeed 2-filling. On the other hand, suppose $\Sigma$ had three elements in the grand splitting, and $L_{2}=C_{1}\cup C_{2}\cup l$ where $C_{1}$ and $C_{2}$ are connected components of $L_{2}$ disjoint from a common witness and $l$ is asymptotic to $C_{1}$ and $C_{2}$. Then since $\mathrm{supp}\left(L_{2}\right)$ is a witness, $C_{1}$ and $C_{2}$ must each separate an element of the grand splitting from the rest. Let $l'$ be an isolated leaf asymptotic to $C_{1}$ on one side, disjoint from $l$ and converging to a maximal end in the third element of the grand splitting. Then $L'=C_{1}\cup l'$ is a 1-filling lamination (to construct a grand arc disjoint from $L'$, follow along $l'$ to the first point of $l'\cap l$ along $l'$, then converge to a maximal end separated by $C_{2}$) disjoint from $L_{2}$, proving again that $L_{2}$ is at most $2$-filling. 

Now for the $\implies$ direction, suppose $L_{2}$ is 2-filling. Then $\mathrm{supp}(L_{2})$ must be a witness, and there exists some 1-filling lamination $L_{1}$ disjoint from $L_{2}$. Since $\mathrm{supp}\left(L_{1}\right)$ is a partial witness (by Lemma \ref{lem:1-filling}), it must intersect $\mathrm{supp}\left(L_{2}\right)$ essentially. Let $M$ be the smallest subsurface of $\Sigma$ containing some connected component $L'\subset L_{1}\cap L_{2}$. Note that $M$ is not a witness, since $\mathrm{supp}\left(L_{1}\right)\supset M$. Also since $L_{1}\pitchfork L_{2}=\phi$, they're asymptotic to each other inside $M$. Thus there is a common sublamination $L'\subset M$ of $L_{1}$ and $L_{2}$. This sublamination fills $M$ (since $L_{1}$ and $L_{2}$ each fill $M$). So if $M$ is a partial witness, then $L'$ must be 1-filling (again by Lemma \ref{lem:1-filling}). This is the desired sublamination of $L_{2}$. 

Now, suppose $M$ is not a partial witness (i.e. $M$ is disjoint from some witness $W$). Since $\mathrm{supp}\left(L_{2}\right)$ is a witness, for each element $m_{i}$ of the grand splitting, there exists a separating simple closed curve $\gamma_{i}\subset\mathrm{supp}\left(L_{2}\right)\cup\partial\mathrm{supp}\left(L_{2}\right)$ which separates $m_{i}$ from the rest of the elements of the grand splitting. Let $W_{0}$ denote a compact witness in $\Sigma$ whose boundary is given by the curves $\gamma_{i}$ (plus some curves corresponding to non-maximal ends, if any). Up to choosing a bigger compact witness $W_{0}\subset\mathrm{supp}\left(L_{2}\right)$, assume that $W_{0}\cap M\neq\phi$ (we can do this since $\mathrm{supp}\left(L_{2}\right)$ is connected). 

Now inductively, pick a leaf $l\in L_{2}$ which accumulates to $L'$ on one side, and is contained in $W_{0}$. Consider the lamination $L''=\overline{L'\cup l}$. Suppose that $\mathrm{supp}\left(L''\right)$ is a witness. In this case, either $l$ accumulates to $L'$ on one side and a witness-filling lamination on the other side, or $\Sigma$ has 3 elements in the grand splitting and $l$ accumulates to two components $L'$ and $C_{2}$ each disjoint from a witness and separating an element of the grand splitting from the rest. \textcolor{red}{Or $l$ accumulates to a partial witness and $L'$ separates one end. In this case we have a 1-filling sublamination too.} 

In the latter case, we're done. \textcolor{red}{Just handle the 3 ends case separately.} \textcolor{blue}{If there were two components of $L_1\cap L_2$ both cutting off different max ends, then we can find a grand arc}

In the former case, note that $\mathrm{supp}\left(L_{1}\right)\pitchfork\mathrm{supp}\left(L''\right)\neq\phi$ since $L_{1}$ is $1$-filling. So $L_{1}$ and $L''$ have a common non-trivial sublamination $M'$ supported on the subsurface where their supports intersect. Since a single leaf can only accumulate to at most two sublaminations, the only possibility is that $l$ is an isolated leaf accumulating to $L'$ and $M'$. As before, if $S$ is 1-filling, then we're done. Else, $S$ is also disjoint from a witness, so $L''$ can be at most 1-filling. \textcolor{red}{I think $S$ is $L'\cup l\cup M'$.}

On the other hand, if $\mathrm{supp}(L'')$ is not a witness, then we continue this procedure, inductively adding leaves of $L_2$ contained in $W_0$ and taking the closure to form a sequence of sublaminations $L^{(i)}$.
%In conclusion, we can consider larger and larger sublaminations of $L_{2}$, each obtained from the previous one by adding a leaf of $W_{0}$ and taking its closure. 
Since $W_{0}$ is compact, this process teminates at a finite step $k$.  If $\Sigma$ has at least 4 elements in the grand splitting, then at this step we have found a 1-filling sublamination $L^{(k)}$ of $L_2$.  If $\Sigma$ has 3 elements in the grand splitting, then at this step we have found a sublamination of the desired form.
%either $\supp\left(L^{(k)}\right)$ is a partial witness, in which case....., or $L^{(k)}$ is a 1-filling sublamination of $L_{2}$. 
\end{proof}

\begin{cor}\label{cor:no-3-filling}
Any lamination transversely disjoint from a 2-filling lamination is at most 2-filling. In particular, there are no $k$-filling laminations for any $k\geq3$. 
\end{cor}

\begin{proof}
Suppose $L_{2}$ is a $2$-filling lamination, and $K$ is any lamination with $K\pitchfork L_{2}=\phi$. By Lemma \ref{lem:2-filling laminations}, there exists a 1-filling sublamination $L_{1}\subset L_{2}$. But then $K\pitchfork L_{1}=\phi$, so $K$ is at most 2-filling. Thus, there cannot be any $k$-filling laminations for $k\geq3$.
\end{proof}
%

\textcolor{red}{Rewrite this for surfaces with 3 max ends, or just assume everything has 4 max ends?}

In summary, we have the following classification of grand laminations - a grand lamination $L$ is: 
\begin{enumerate}
\item 0-filling, if $L$ is a single grand arc.
\item 1-filling, if $\mathrm{supp}(L)$ is a partial witness which is not a single infinite rectangular strip.
\item 2-filling, if $\mathrm{supp}(L)$ is a witness, and $L$ has a 1-filling sublamination.
\item High-filling otherwise ($\mathrm{supp}(L)$ is a witness and $L$ does not have a 1-filling sublamination). 
\end{enumerate}

\subsection{The connected component containing grand arcs}

Assume for now that $\Sigma$ has at least 4 elements in its grand splitting. As defined earlier, let $\overline{\mathcal{G}}_{0}\left(\Sigma\right)$ be the connected component of $\overline{\mathcal{G}}\left(\Sigma\right)$ consisting of all the grand arcs (hence all the $k$-filling grand laminations as well). In this section, we shall prove the first part of Theorem \ref{thm:completed_graph_qi}, that $\overline{\mathcal{G}}_{0}\left(\Sigma\right)$ is quasi-isometric to $\mathcal{G}\left(\Sigma\right)$. The proof proceeds in two steps. First, we show that for any two grand arcs, there must be a geodesic in $\overline{\mathcal{G}}\left(\Sigma\right)$ that does not have any 2-filling laminations. Second, we show (in the Lemma below) that for any geodesic between grand arcs consisting of 1-filling laminations, there exists a uniform quasi-geodesic consisting only of grand arcs.

\begin{lem}
\label{lem:length_3_paths}Let $a,b\in\mathcal{G}\left(\Sigma\right)$ and suppose that $d_{\overline{\mathcal{G}}}\left(a,b\right)\leq3.$Then $d_{\mathcal{G}}\left(a,b\right)\leq3$.
\end{lem}

\begin{proof}
The cases when $d_{\overline{\mathcal{G}}}\left(a,b\right)\leq1$ are trivial. Suppose $d_{\overline{\mathcal{G}}}\left(a,b\right)=2$, and there is a path $a-L-b$ for some $L\in\Lambda_{\mathcal{G}}$. Then $L$ is 1-filling, so $Y=\mathrm{supp}\left(L\right)$ is a partial witness (by Lemma \ref{lem:1-filling}. Moreover, $a,b$ must intersect each other, so they lie in the same component of $\Sigma\backslash Y$. Since $Y$ is a partial witness, we can find a grand arc $c$ that is disjoint from this component (else this component would be a witness of $\mathcal{G}\left(\Sigma\right)$ disjoint from $Y$). This grand arc $c$ is disjoint from $a,b$, so that $d_{\mathcal{G}}\left(a,b\right)=2$. 

Now, suppose that $d_{\mathcal{\overline{G}}}\left(a,b\right)=3.$ So there exist laminations $L_{1},L_{2}\in\Lambda_{\mathcal{G}}$ such that 
\[
a-L_{1}-L_{2}-b.
\]
Also assume that $d_{\mathcal{G}}\left(a,b\right)\geq3$ (else we're already done). Then we can pick a compact witness $W$ such that $a\cap W$ and $b\cap W$ are connected. Note that $d_{W}\left(a,b\right)\geq3$ as well, so that $a,b$ fills $W$. Then for $i=1,2$, $L_{i}\cap W$ may consist of simple arcs joining different components of $\partial W$, or arcs starting at a component of $\partial W$ and accumulating to a sublamination in $W$, or geodesics contained in $W$. If either $L_{1}$ (respectively, $L_{2}$) is completely contained inside $W$, then add geodesics asymptotic to $L_{1}$ (respectively, $L_{2}$) and converging to maximal ends, whilst staying disjoint from $a$ (respectively, $b$). This way, both $L_{1}\cap W$ and $L_{2}\cap W$ must intersect at least two boundary components of $W$, corresponding to distinct elements of the grand splitting. 

Suppose $L_{1}\cap W$ (along with $\partial W$) connects two boundary curves $\gamma_{1}$ and $\gamma_{2}$, which separate two distinct elements of the grand splitting. If $L_{1}\cap W$ contains a proper arc connecting $\gamma_{1}$ and $\gamma_{2}$, we can complete it to a grand arc $c$ which stays disjoint from $a$. Else, if $L_{1}\cap W$ contains a sublamination connecting $\gamma_{1}$ and $\gamma_{2}$, we can choose an embedded arc $\beta$ contained in the support of this sublamination, which connects these boundary components (and extend it to a grand arc $c$ as before). Finally, if any path in $L_{1}\cap W$ connecting $\gamma_{1}$ and $\gamma_{2}$ passes through other boundary components of $W$, then we can add (the closure of) finitely many leaves of $L_{1}$ to $W$ (since $L_{1}$ is connected), to get a bigger compact witness (which we also name $W$) where $L_{1}\cap W$ has a sublamination connecting $\gamma_{1}$ and $\gamma_{2}$. 

Thus, in any case, we can find a grand arc $c$ contained in $\mathrm{supp}\left(L_{1}\right)$, which is disjoint from $a$. Similarly, we can find a grand arc $d$ in $\mathrm{supp}\left(L_{2}\right)$ which stays disjoint from $b$. \textcolor{red}{Pause - be careful in checking that $c$ and $d$ are disjoint.} Since $L_{1}\pitchfork L_{2}=\phi$, we get that 
\[
a-c-d-b,
\]
so that $d_{\mathcal{G}}\left(a,b\right)\leq3$ as desired.
\end{proof}
%
\begin{cor}
The connected component $\overline{\mathcal{G}}_{0}\left(\Sigma\right)$ of $\overline{\mathcal{G}}\left(\Sigma\right)$ consisting of all the grand arcs is quasi-isometric to $\mathcal{G}\left(\Sigma\right)$. 
\end{cor}

\begin{proof}
We shall show the inclusion $\mathcal{G}\left(\Sigma\right)\hookrightarrow\overline{\mathcal{G}}\left(\Sigma\right)$ is a quasi-isometry. This is clearly coarsely surjective, since any $k$-filling grand lamination is actually at most 2-filling. Moreover, note that $d_{\overline{\mathcal{G}}}\left(a,b\right)\leq d_{\mathcal{G}}\left(a,b\right)$ since any path in $\mathcal{G}\left(\Sigma\right)$ is also a path in $\overline{\mathcal{G}}\left(\Sigma\right)$. Suppose $a,b\in\mathcal{G}\left(\Sigma\right)$, and let $d_{\overline{\mathcal{G}}}\left(a,b\right)=k$. Then there exists a path 
\[
a-L_{1}-\dots-L_{k-1}-b
\]
where each $L_{i}\in\overline{\mathcal{G}}\left(\Sigma\right)$. We shall show that $d_{\mathcal{G}}\left(a,b\right)\leq3k$. 

First, note that each $L_{i}$ is at most 2-filling. If $L_{i}$ is 1-filling, set $M_{i}=L_{i}$. Else, $L_{i}$ has a 1-filling sublamination (by Lemma \ref{lem:2-filling laminations}); call this sublamination $M_{i}$. Then $M_{i}$ is (transversely) disjoint from $L_{i-1}$ and $L_{i+1}$, so that 
\[
M_{i-1}-M_{i}-M_{i+1}
\]
is still a path in $\overline{\mathcal{G}}\left(\Sigma\right)$. Thus, we get a path 
\[
a-M_{1}-\dots-M_{k-1}-b
\]
in $\overline{\mathcal{G}}\left(\Sigma\right)$, which must be a geodesic since it's the correct length. So, we may in fact assume that each $L_{i}$ is 1-filing. 

So, for each $i=2,\dots,k-2$, there exists a grand arc $x_{i}$ disjoint from $L_{i}$. Set $x_{1}=a$ and $x_{k-1}=b$. Then for each $i=1,\dots,k-2$, we have a path 
\[
x_{i}-L_{i}-L_{i+1}-x_{i+1}
\]
in $\overline{\mathcal{G}}\left(\Sigma\right)$, so that $d_{\overline{\mathcal{G}}}\left(x_{i},x_{i+1}\right)\leq3$. By Lemma \ref{lem:length_3_paths}, in fact $d_{\mathcal{G}}\left(x_{i},x_{i+1}\right)\leq3$. Thus, $d_{\mathcal{G}}\left(a,b\right)\leq3\cdot d_{\overline{\mathcal{G}}}\left(a,b\right)$. Thus, the inclusion $\mathcal{G}\left(\Sigma\right)\hookrightarrow\overline{\mathcal{G}}\left(\Sigma\right)$ is a quasi-isometric embedding, and hence a quasi-isometry.
\end{proof}

\subsection{Connected components of high-filling laminations}

Denote $\mathcal{HF}\left(\Sigma\right)$ to be the subspace of $\Lambda\left(\Sigma\right)$ (with the coarse Chabauty topology) consisting of the high-filling laminations. Denote $\mathcal{CHF}\left(\Sigma\right)$ to be the quotient of $\mathcal{HF}\left(\Sigma\right)$, by the relation $L_{1}\sim L_{2}$ if $L_{1}$ and $L_{2}$ are in the same connected component of $\overline{\mathcal{G}}\left(\Sigma\right)$. Let $q:\mathcal{HF}\left(\Sigma\right)\to\mathcal{CHF}\left(\Sigma\right)$ denote this quotient map. In this subsection, we shall gather evidence why $\mathcal{CHF}\left(\Sigma\right)$ could be a reasonable candidate for ``a space of laminations homeomorphic to $\partial\left(\mathcal{G}\left(\Sigma\right)\right)$". 
\begin{lem}
$\mathcal{CHF}\left(\Sigma\right)$ with the (quotient coarse Chabauty topology) is Hausdorff.
\end{lem}

\begin{proof}
\textcolor{red}{INCOMPLETE} First, note that $\mathcal{HF}\left(\Sigma\right)$ is first-countability - this follows from the first-countability of $\Lambda\left(\Sigma\right)$ with the coarse Chabauty topology, and the fact that subspaces of first-countable spaces are first-countable. Hence, $\mathcal{HF}\left(\Sigma\right)$ is a sequential space. As a quotient of $\mathcal{HF}\left(\Sigma\right)$, this implies that $\mathcal{CHF}\left(\Sigma\right)$ is also a sequential space. Thus, showing that $\mathcal{CHF}\left(\Sigma\right)$ is Hausdorff is equivalent to showing that it is sequentially Hausdorff, that is, every convergent sequence has a unique limit point. 

Suppose $\left(X_{n}\right)_{n\in\mathbb{N}}$ is a sequence in $\mathcal{CHF}\left(\Sigma\right)$, such that ... Either need some combinatorial info (that connected comps are finite diameter) or some geometric info (that the laminations are close somehow). Plus, $\mathcal{HF}\left(\Sigma\right)$ with the coarse Chabauty topology isn't Hausdorff.
\end{proof}

\begin{rem}
Special case - when $\Sigma=\mathbb{R}^{2}\backslash\mathrm{Cantor}$, we will get that $\mathcal{CHF}\left(\Sigma\right)$ is Hausdorff.
\end{rem}

Next, we shall show that $\mathcal{GEL}\left(\Sigma\right)$ is a subspace of $\mathcal{CHF}\left(\Sigma\right)$. 
\begin{lem}
\label{lem:GEL_high-filling}Let $L\in\mathcal{GEL}\left(\Sigma\right)$. Then $L$ is a high-filling lamination. Moreover, any lamination in the connected component $q(L)$ of $L$ in $\overline{\mathcal{G}}\left(\Sigma\right)$ must contain $L$ as a sublamination. 
\end{lem}

\begin{proof}
Suppose there were a finite path 
\[
X_{1}-X_{2}-\dots-X_{k}-L
\]
in $\overline{\mathcal{G}}\left(\Sigma\right)$ between some grand lamination $X_{1}$ and $L$. Using Lemma \ref{lem:sublamination} repeatedly, we get that each $X_{i}$ must have $L$ as a sublamination. This proves the second assertion. In particular, since a single grand arc doesn't fill a witness, it cannot have $L$ as a sublamination. So, $L$ is disconnected from any grand arc, and must be high-filling.
\end{proof}
%
\begin{question}
Is $\mathcal{GEL}\left(\Sigma\right)=\mathcal{HF}\left(\Sigma\right)$?
\end{question}

\begin{cor}
Let $L\in\mathcal{GEL}\left(\Sigma\right)$. Then $\mathrm{diam}_{\overline{\mathcal{G}}\left(\Sigma\right)}\left(q(L)\right)\leq2$.
\end{cor}

\begin{proof}
Suppose $L_{1},L_{2}$ are two grand laminations in $q(L)$. Then by \ref{lem:GEL_high-filling}, both $L_{1}$ and $L_{2}$ must have $L$ as a sublamination. Thus, 
\[
L_{1}-L-L_{2}
\]
is a length $2$ path in $\overline{\mathcal{G}}\left(\Sigma\right)$ between $L_{1}$ and $L_{2}$. 
\end{proof}
%
Since both $\mathcal{GEL}\left(\Sigma\right)$ and $\mathcal{HF}\left(\Sigma\right)$ are subspaces of $\Lambda\left(\Sigma\right)$ with the coarse Chabauty topology, and $\mathcal{GEL}\left(\Sigma\right)$ is a subset of $\mathcal{HF}\left(\Sigma\right)$ by Lemma \ref{lem:GEL_high-filling}, it follows that $\mathcal{GEL}\left(\Sigma\right)$ is a subspace of $\mathcal{HF}\left(\Sigma\right)$. 
\begin{lem}
The map $q\mid_{\mathcal{GEL}\left(\Sigma\right)}:\mathcal{GEL}\left(\Sigma\right)\to\mathcal{CHF}\left(\Sigma\right)$ (interpreting $\mathcal{GEL}\left(\Sigma\right)$ as a subspace of $\mathcal{HF}\left(\Sigma\right)$) is an embedding.
\end{lem}

\begin{proof}
It suffices to show that $q\mid_{\mathcal{GEL}\left(\Sigma\right)}$ is injective. Suppose $L_{1},L_{2}\in\mathcal{GEL}\left(\Sigma\right)$ with $q\left(L_{1}\right)=q\left(L_{2}\right)$. Then by Lemma \ref{lem:GEL_high-filling}, $L_{1}$ must have $L_{2}$ as a sublamination (and vice-versa). Since $L_{1}$ is minimal, it follows that $L_{1}=L_{2}$. 
\end{proof}
%
We shall now focus on the special case, when $\Sigma$ is the once-punctured Cantor tree. Following the terminology in \cite{B-W}, we shall prove that the space $\mathcal{CHF}\left(\Sigma\right)$ is homeomorphic to the space of connected components of high-filling rays. This also implies that $\mathcal{CHF}\left(\Sigma\right)\cong\partial\left(\mathcal{G}\left(\Sigma\right)\right)$.


==> Modules/Finite_Bicorns.tex <==
\section{Bicorn arcs in $\mathcal{G}(\Sigma)$} 

\textcolor{red}{UPDATE - I want to redo this section so that unicorns aren't bicorns.}

Given two proper geodesics $a,b$ on $\Sigma$, their intersection $a\cap b$ is a discrete (possibly infinite) collection of points.  We will use these intersection points to build new prescribed arcs.

Previously, Bar-Natan and Verberne (see \cite{B-NV}) and Kopreski (see \cite{Kop}) construct \textit{unicorn arcs} to study the geometry of the grand arc graph and prescribed arc graphs respectively. Unicorn arcs were defined in the finite-type setting by \cite{HPW} and extended to the infinite-type setting by \cite{F-G-M}. A unicorn arc between $a$ and $b$ is a simple arc of the form $x=a'\cup b'$, where $a', b'$ are the closures of components of $a\setminus\{P\}$ and $b\setminus \{P\}$ for a point $P\in a\cap b$.  Note that $x$ is only  simple when $a'\cap b'=\{P\}$, hence not every point of intersection of $a$ and $b$ will define a unicorn arc. We denote the set of unicorn arcs between $a$ and $b$ by $\mc U(a,b)$. Note that $a,b\in \mc U(a,b)$ and $\mc U(a,b)=\mc U(b,a)$. A unicorn arc in $\mc U(a,b)\setminus\{a,b\}$ is called a \textit{proper unicorn arc}.  We define a larger class of arcs between $a$ and $b$ which we call \textit{bicorn arcs}.

\begin{defn}
A \textit{bicorn arc between grand arcs $a$ and $b$} is a grand arc of the type $x=a_{1}\cup b_{1}\cup a_{2}$, where $a_{1},a_{2}\subset a$ are the closures of the unbounded components of $a\setminus\{P,Q\}$ and $b_{1}\subset b$ is the closure of a component of $b\setminus \{P,Q\}$, where $P,Q\in a\cap b$.  We allow any of $a_i,b_1$ to be empty.  As for unicorn arcs, this is only a simple arc if $(a_1\cup a_2)\cap b_1=\{P,Q\}$.  Denote  the collection of bicorns arcs between $a$ and $b$ by $\mathcal{B}\left(a,b\right)$. Since we allow some of $a_i,b_1$ to be empty, the unicorn arcs $\mathcal{U}(a,b)$ are also bicorn arcs. In particular,  $a,b\in\mathcal{B}\left(a,b\right)$.  If $x=a_1\cup b_1\cup a_2$ is not a unicorn arc, that is, if $b_1$ is a non-empty subsegment of $b$ of finite length, then we say $x$ is a \textit{proper bicorn arc}.
\end{defn} 

If $x_1$ is a compact subsegment of an arc $x$ and the endpoints of $x_1$ are $P,Q$, we write $x_1\equiv (PQ)_x$, meaning that $x_1$ is formed by traveling from the point $P$ to the point $Q$ along the arc $x$.  If $x_1$ is a subsegment of $x$ starting at an end of $x$ and ending at a point $P\in x$, then we write $x_1\equiv (\dots P)_x$.


\begin{figure}[h]
    \centering
    \def\svgwidth{10 cm}
    \import{Pictures}{bicorns_disconnected.pdf_tex}
    \captionsetup{margin=1.5 cm, justification=justified, singlelinecheck=false}
    \caption{Every bicorn between the grand arcs $a$ and $b$  intersects $b$ infinitely many times. It follows that there is no path from $a$ to $b$ in $\mathcal{B}\left(a,b\right)$.}
    \label{fig:bicorns_disconnected}
\end{figure}

In these definitions, $(a,b)$ is an ordered pair, and a priori $\mathcal{B}(a,b)\neq \mathcal{B}(b,a)$. Moreover, $\mathcal{B}\left(a,b\right)$ is not necessarily connected as a subset of $\mathcal{G}(\Sigma)$; for example, see Figure \ref{fig:bicorns_disconnected}. However, similar to \cite[Lemma~5.6]{B-NV}, the $1$-neighbourhood of $\mathcal{B}\left(a,b\right)$ is connected.

\begin{lem}\label{lem:finite_bicorns_connected}
For any $a,b\in\mathcal{G}\left(\Sigma\right)$, the $1$-neighbourhood $N_{1}\left(\mathcal{B}\left(a,b\right)\right)$ of $\mathcal{B}\left(a,b\right)$ in $\mathcal{G}\left(\Sigma\right)$ is connected.
\end{lem}

\begin{proof}
Since the 1-neighbourhood of the unicorn paths $N_{1}\left(\mathcal{U}\left(a,b\right)\right)$ is connected \cite[Lemma~5.6]{B-NV}, it suffices to show that there is a path in $N_{1}\left(\mathcal{B}\left(a,b\right)\right)$ from any proper bicorn arc $x$ to $a$. 

\begin{figure}[h]
    \centering
    \includegraphics[width=12 cm]{Pictures/bicorn_connected.pdf}
    \caption{Constructing a path from $x$ to $a$.}
    \label{fig:bicorns_connected}
\end{figure}

Since $x$ is a proper bicorn arc, $b_{1}$ is a segment of finite length along $b$, so $a\cap b_{1}=a\cap x$ is a finite set. %Since $a\cap b_{1} = a\cap x$, it follows that $a\cap x$ is finite, as well. 
We induct on the number of points of $a\cap x$. If $a\cap x=\emptyset$, then the path $a-x$ is in $N_{1}\left(\mathcal{B}\left(a,b\right)\right)$. Now, suppose the statement is true for all $y\in\mathcal{B}\left(a,b\right)$ with $\#a\cap y\leq n$, and suppose $x$ is a bicorn arc with $\#a\cap x=n+1$. Let $x=a_{1}\cup b_{1}\cup a_{2}$, with $b_{1}=\left(PQ\right)_{b}$. Orient $a$ from $P$ towards $Q$, and consider the first point of intersection $R$ of $\left(PQ\right)_{a}\cap b_{1}$ along $a$.  Note that $\left(PQ\right)_{a}$ may intersect $b$ outside $b_{1}$, but we are not concerned with those intersections. Then $x'=\left(a_{1}\cup\left(PR\right)_{a}\right)\cup\left(RQ\right)_{b}\cup a_{2}$ is a bicorn such that $\# a\cap x' < \# a \cap x$, and $\#x\cap x'\leq1$; see Figure \ref{fig:bicorns_connected}. By induction, there is a path in $N_{1}\left(\mathcal{B}\left(a,b\right)\right)$ between $a$ and $x'$. If $\#x\cap x'=0$, then they are connected by an edge.  If $\#x\cap x'=1$, then by taking a proper unicorn path $c$  between $x$ and $x'$, we obtain a path $x-c-x'$ in $N_{1}\left(\mathcal{B}\left(a,b\right)\right)$.  In either case, we have found a path from $a$ to $x$ in $N_{1}\left(\mathcal{B}\left(a,b\right)\right)$, completing the proof. 
\end{proof}

\begin{lem}\label{lem:finite_bicorn_subset}
If $a,b\in\mathcal{G}\left(\Sigma\right)$ and $x\in\mathcal{B}\left(a,b\right)$, then $\mathcal{B}\left(a,x\right)\subset\mathcal{B}\left(a,b\right)$. 
\end{lem}

\begin{proof}
Suppose $x=a_{1}\cup b_{1}\cup a_{2}$ is a bicorn arc; we allow $a_2$ to be empty. Any point of $a\cap x$ is a point of $a\cap b_{1}\subseteq a\cap b$, and so any bicorn arc between $a$ and $x$ is necessarily a bicorn arc between $a$ and $b$.
\end{proof}

Changing one arc used to build unicorn arcs to an adjacent arc does not have a large effect on the unicorn set:

\begin{lem} \label{lem:unicorns_changing_first_arc}
If $a,a'\in\mathcal{G}\left(\Sigma\right)$ are disjoint and $b\in\mathcal{G}\left(\Sigma\right)$, then, as subsets of $\mathcal{G}\left(\Sigma\right)$, \[d_{\mathrm{Haus}}\left(\mathcal{U}\left(a,b\right),\mathcal{U}\left(a',b\right)\right)\leq1.\]
\end{lem}

\begin{proof}
Let $p=a_{1}\cup b_{1}=(\dots P)_{a}\cup (P\dots)_b$ be a unicorn arc in $\mathcal{U}\left(a,b\right)$, oriented so that $b_1$ is oriented away from $P$. If $\mathcal{U}\left(a',b\right)= \{ a',b\} $, the result is trivially true, so suppose this is not the case.  We will construct a unicorn arc $q\in\mathcal{U}\left(a',b\right)$ disjoint from $p$. First, note that any point of $a'\cap p$ is a point of $a'\cap b_{1}$. %Not all points of $a'\cap b_{1}$ define unicorn arcs. 
Let $Q\in a'\cap b_{1}$ be the closest point to $P$ along $b_{1}$ that defines a unicorn arc.  Such a point $Q$ exists as we have assumed that $\mathcal{U}\left(a',b\right) \neq \{ a',b\} $ By construction, $q=\left(\dots Q\right)_{a'}\cup\left(Q\dots\right)_{b_{1}}$ is a unicorn arc between $a'$ and $b$ that is disjoint from $p$. See Figure \ref{fig:unicorns_first_change}.
\end{proof}

\begin{figure}
    \centering
    \includegraphics[width=12 cm]{Pictures/unicorns_first_change.pdf}
    \caption{Constructing a unicorn arc in $\mathcal{U}\left(a',b\right)$ disjoint from $p$.}
    \label{fig:unicorns_first_change}
\end{figure}



We next show an analogue of \Cref{lem:unicorns_changing_first_arc} for the set of bicorn arcs.

\begin{lem} \label{lem:bicorn_changing_first_arc}
If $a,a'\in\mathcal{G}\left(\Sigma\right)$ are disjoint and $b\in\mathcal{G}\left(\Sigma\right)$, then, as subsets of $\mathcal{G}\left(\Sigma\right)$, \[d_{\mathrm{Haus}}\left(\mathcal{B}\left(a,b\right),\mathcal{B}\left(a',b\right)\right)\leq2.\]
\end{lem}

\begin{proof}
Let $p=a_{1}\cup b_{1}\cup a_{2}\in \mc B(a,b)$ be a bicorn arc, with $a_{2}$ possibly empty if $p$ is a unicorn arc. We will construct $q\in\mathcal{B}\left(a',b\right)$ such that $d_{\mathcal{G}}\left(p,q\right)\leq2$. If $\#a'\cap b_{1}\leq1$, then setting $q=a'$ completes the proof.  To see this, note that if $a'\cap b_1=\emptyset$, then $d_{\mc G}(a',p)=1$, while if $\#a'\cap b_1=1$, then there is a unicorn path between $a'$ and $p$ disjoint from both $a'$ and $p$, so $d_{\mc G}(a',p)\leq 2$.\carolyn{We use this same argument at least twice.  Maybe it should be a quick lemma?  Let's see how many more times we use it.}  

On the other hand, suppose $\#a'\cap b_1 \geq 2$.  Pick an orientation on $a'$, and let $X,Y$ denote the first and last points of $a'\cap b_{1}$ along $a'$, respectively. Then $q=\left(\dots X\right)_{a'}\cup\left(XY\right)_{b_{1}}\cup\left(Y\dots\right)_{a'}$ is a bicorn arc in $\mathcal{B}\left(a',b\right)$ which intersects $p$ in at most one point. It follows $d_{\mathcal{G}}\left(p,q\right)\leq2$, as in the previous paragraph. See Figure \ref{fig:bicorns_first_change}.
\end{proof}

\begin{figure}[h]
    \centering
    \includegraphics[width=12 cm]{Pictures/bicorns_first_change.pdf}
    \caption{Constructing a bicorn arc in $\mathcal{B}\left(a',b\right)$ disjoint from $p$.}
    \label{fig:bicorns_first_change}
\end{figure}



We next show that the set $N_{1}\left(\mathcal{B}\left(a,b\right)\right)$ is an unparametrized quasi-geodesic from $a$ to $b$. To see this, we invoke the Guessing Geodesics Lemma.

\begin{lem}[Guessing Geodesics Lemma, {\cite{M-S}}]
Suppose $G$ is a connected graph and for each $x,y\in V(G)$ there is an associated connected subgraph $A\left(x,y\right)$ with $x,y\in A\left(x,y\right)$. Suppose there is a uniform constant $h>0$ such that the following hold.
\begin{enumerate}
\item For any $x,y,z\in V(G)$, 
\[
A\left(x,y\right)\subset N_{h}\left(A\left(x,z\right)\cup A\left(z,y\right)\right).
\]
\item For any $x,y\in V(G)$ with $d\left(x,y\right)\leq1$, the diameter of $A\left(x,y\right)$ in $G$ is at most $h$. 
\end{enumerate}
Then $G$ is hyperbolic. Moreover, there is a uniform constant $m>0$ such that 
\[
d_{\mathrm{Haus}}\left(A\left(x,y\right),\left[x,y\right]\right)\leq m,
\]
where $\left[x,y\right]$ denotes any geodesic between $x$ and $y$ in $G$. 
\end{lem}

We will apply the Guessing Geodesics Lemma with $A(x,y)=N_1(\mathcal B(x,y))$ for grand arcs $x,y$, which is a connected subgraph by Lemma~\ref{lem:finite_bicorns_connected}.  We first show that the first condition holds. 

\begin{lem}\label{lem:ApplyGG}
Suppose $\Sigma$ is an infinite-type surface with at least $3$ maximal end types. If $a,b,c\in\mathcal{G}\left(\Sigma\right)$, then $A\left(a,b\right)\subseteq N_{3}\left(A\left(a,c\right)\cup A\left(b,c\right)\right)$, where $A\left(x,y\right)= N_{1}\left(\mathcal{B}\left(x,y\right)\right)$ for $x,y\in\mathcal{G}\left(\Sigma\right)$. 
\end{lem}

\begin{proof}
It is shown in \cite[Lemma~5.8]{B-NV} that $N_{1}\left(\mathcal{U}\left(a,b\right)\right) \subset N_{3}\left(N_{1}\left(\mathcal{U}\left(a,c\right)\right)\cup N_{1}\left(\mathcal{U}\left(b,c\right)\right)\right)$, and so it remains to consider proper bicorns.  We will show that $\mathcal B(a,b)\subseteq N_1(A(a,c)\cup A(b,c))$, which will then imply that $A(a,b)\subseteq N_3(A(a,c)\cup A(b,c))$.  The remainder of the proof closely follows that of \cite[Lemma~6.1]{F-G-M}.

Suppose $x=a_1\cup b_1\cup a_2\in\mathcal{B}\left(a,b\right)$ is a proper bicorn, where $a_1,a_2\subset a$ and $b_1\subset b$. Our goal is to find and arc $y\in A(a,c)\cup A(b,c)$ with $d(x,y)\leq 1$.  If $x\cap c=\emptyset$, then we can take $y=c\in \mc U(a,c)\subseteq A(a,c)$, %then $d_{\mathrm{Haus}}\left(\left\{ x\right\} ,\mathcal{U}\left(a,c\right)\cup\mathcal{U}\left(b,c\right)\right)\leq1$\carolyn{I see that in this case the always exists a unicorn in $\mc U(a,c) \cup \mc U(b,c)$ that is disjoint from $x$, but it seems there are also ones that intersect $x$.  We don't need a staetment about Hausdorff distance, though.  I think here we just want that $x\in \mc N_1(\mathcal{U}\left(a,c\right)\cup\mathcal{U}\left(b,c\right)$.  Similarly for the next sentence.}, and so $d_{\mathrm{Haus}}\left(A\left(a,b\right),A\left(a,c\right)\cup A\left(b,c\right)\right)\leq3$. 
so assume $\#x\cap c\geq1$. 

First, suppose $c$ converges to a maximal end class $e$ to which $a$ does not converge. Orient $c$ away from $e$, and follow along $c$ to the first point of intersection $P$ with $x$; a first such point exists, because $x$ does not converge to $e$. Up to homotopy, we can assume that $P\in a$, and up to re-orienting $x$, we can assume $P\in a_1$. Consider the grand arc $y$ obtained by traveling along $c$ to $P$, then following $a_1$. Then $y\in\mathcal{U}\left(c,a\right)=\mathcal{U}\left(a,c\right)\subseteq A(a,c)$, and $x$ and $y$ are disjoint. 

Finally, suppose $c$ and $a$ have the same ends. Then there exists a grand arc $d$ which is disjoint from $c$, and converges to a maximal end to which $a$ does not converge: start with any grand arc $d'$ starting at a maximal end to which $a$ does not converge, and construct $d$ by following $d'$ to the first point of intersection with $c$ and then following $c$.  In this case, the arguments of the previous paragraph construct an arc  $y\in\mathcal{U}\left(d,a\right)$ which is disjoint from $x$. Since $d\cap c=\emptyset$, Lemma~\ref{lem:unicorns_changing_first_arc} implies that $d_{\mathrm{Haus}}\left(\mathcal{U}\left(d,a\right),\mathcal{U}\left(c,a\right)\right)\leq1$, and so $y\in N_{1}\left(\mathcal{U}\left(c,a\right)\right)\subseteq A\left(a,c\right)$, completing the proof. 
\end{proof}

We are now able to obtain a new proof that the grand arc graph is hyperbolic if the surface has at least three maximal end types. 

\carolyn{Changed $m$ to $M_0$.}
\begin{cor}\label{cor:unicorn_hausdorff_dist}
If $\Sigma$ is an infinite-type surface with at least $3$ elements in the grand splitting, then the grand arc graph $\mathcal{G}\left(\Sigma\right)$ is $\delta$-hyperbolic. Moreover, there is a uniform constant $M_0>0$ such that for any $x,y\in\mathcal{G}\left(\Sigma\right)$ and any geodesic $\left[x,y\right]$ between $x$ and $y$ in $\mathcal{G}\left(\Sigma\right)$, we have 
\[
d_{\mathrm{Haus}}\left(\mathcal{B}\left(x,y\right),\left[x,y\right]\right)\leq M_0.
\] 
\end{cor}

\begin{proof}
    We will show that the Guessing Geodesics Lemma holds  with $A(x,y)=N_1(\mathcal B(x,y))$, for grand arcs $x,y$, and $h=3$.  The first condition holds by Lemma~\ref{lem:ApplyGG}.  For the second condition, note that if $x\cap y=\emptyset$, then $\mathcal B(x,y)=\{x,y\}$, a set of diameter 1, and so $A(x,y)=N_1(\mathcal B(x,y))$ has diameter 3.
\end{proof}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%










==> Modules/New_surjectivity.tex <==
\section{New surjectivity via Lvzhou's proof}

\textcolor{red}{Incomplete, will fill in.}

\begin{lem}\label {lem:unbdd_bicorns_high_filling}
Suppose $l\in\Gamma\left(\Sigma\right)$ and $a\in\mathcal{G}\left(\Sigma\right)$. Then $\mathcal{B}\left(a,l\right)$ is unbounded $\iff\overline{l}$ has a minimal component which fills a witness.
\end{lem}

\begin{proof}
We have proved one direction of this statement in \ref{lem:grand_bicorns_go_to_infty}, that if $\overline{l}$ has a minimal component which fills a witness, then $\mathcal{B}\left(a,l\right)$ is unbounded. So assume that $\overline{l}$ has no minimal component which fills a witness. Note that $\overline{l}$ may have $0$, $1$ or $2$ minimal components - $0$ if $l$ is isolated, $1$ if $l$ converges to an end on one side and is asymptotic to a minimal lamination on the other, and $2$ if it is asymptotic to a minimal lamination on both sides. Also note that by Lemma \ref{lem:bicorns_change_base_pt}, if the statement of the theorem holds for some grand arc $a$, it will hold for all of them. 

If $l$ is isolated (i.e. $\overline{l}=l$), then we can find a grand arc intersecting $l$ at most once (since $\Sigma -l$ is a surface).

Next, if $l$ is asymptotic to one minimal component. Then by our assumption, $\mathrm{supp}\left(\overline{l}\right)$ is not a witness, and in particular, is disjoint from some grand arc $b$. Then $\mathcal{B}\left(b,l\right)=\left\{ b\right\} $.

Finally, suppose $l$ is asymptotic to two minimal components $C_{1}$ and $C_{2}$, neither of which fill a witness (but their union might!). Choose grand arcs $b_{1},b_{2}$ such that $b_{i}\cap\mathrm{supp}\left(C_{i}\right)=\phi$ and $b_{1}\cap b_{2}=\phi$. Then any bicorn arc in $\mathcal{B}\left(b_{1},l\right)$ is disjoint from $b_{2}$; so $\mathrm{diam}\left(\mathcal{B}\left(b_{1},l\right)\right)\leq2$. Thus, for any $l\in\Gamma(\Sigma)$, if $\overline{l}$ does not have a minimal witness-filling component, then $\mathcal{B}\left(a,l\right)$ is bounded. 
\end{proof}
%
\begin{rem}
This makes us want to define: $l\in\Gamma\left(\Sigma\right)$ is $0$-filling if $l$ is contained in the complement of some witness; $1$-filling if $l$ intersects every witness but is disjoint from a grand arc; $2$-filling if $l$ intersects every grand arc but $\overline{l}$ has no minimal sublamination which fills a witness, and high-filling if $\overline{l}$ does have a minimal sublamination which fills a witness. Then the above lemma could be restated as ``$\mathcal{B}\left(a,l\right)$ is unbounded if and only if $l$ is high-filling''. 
\end{rem}

\begin{rem}
In the proof of the Lemma above, we can say something stronger - if $l$ not high-filling, then there exists a grand arc $a$ such that $\mathcal{B}(a,l)$ has diameter at most $\sim 2$(?).
\end{rem}

\textcolor{red}{Incomplete, will fill in.}

\begin{proof}[Proof that $\Phi$ is surjective]
Suppose $\left(x_{n}\right)_{n\in\mathbb{N}}$ is a sequence of grand arcs that converges to a point $p$ in $\partial\mathcal{G}\left(\Sigma\right)$. Up to choosing a subsequence, we can assume that $x_{n}\to L$ for some $L\in\Lambda\left(\Sigma\right)$. We shall show that there is a minimal lamination $L_{0}\subset L$ which fills a witness. (Assume/reference here - $x_{n}\to L$ implies $\mathcal{B}\left(a,x_{n}\right)$ agrees with $\mathcal{B}\left(a,x_{m}\right)$ for all $m\geq n$ for finite segments etc.)

To-dos: Show that $\mathcal{B}\left(a,L\right)$ is unbounded. Then by Lemma \ref{lem:unbdd_bicorns_high_filling}, some leaf $l\in L$ must be high-filling. So $\overline{l}$ has a minimal sublamination $L_{0}$ which fills a witness. So $L_{0}\in\mathcal{GEL}\left(\Sigma\right)$ is our candidate inverse for $p$.

First, we show that $\mathcal{B}\left(a,L\right)$ must be unbounded, for any $a\in\mathcal{G}\left(\Sigma\right)$. Suppose otherwise, so that $\mathrm{diam}\left(\mathcal{B}\left(a,L\right)\right)\leq k$. 
\begin{enumerate}
\item Since $\left(x_{i}\right)_{i\in\mathbb{N}}$ is a quasi-geodesic, by Lemma \_\_, there is a $C>0$ (independent of $k$ and $n$) such that for all $n>k$, $\mathcal{B}\left(x_{0},x_{k}\right)$ is contained in a $C$-neighbourhood of $\mathcal{B}\left(x_{0},x_{n}\right)$. 
\item Prove that $\mathrm{supp}(L)$ contains a witness; equivalently, that $L$ doesn't just contain $0$-filling and $1$-filling geodesics. 
\item If $L$ has a $2$-filling geodesic, then we can find a non-boundary leaf of $L$ and do bicorns with this leaf. By non-boundary / both half-leaves being dense, we get a sequence of bicorns which genuinely converges to the leaf, uniformly (in the sense of Lvzhou's proof). 
\item Follow through Lvzhou's proof - the two cases either give us a contradiction to existence of $k$ such that $d\left(b,x_{k}\right)>C$, or to the fact that $\left(x_{k}\right)$ escapes to infinity.
\end{enumerate}
\end{proof}

==> Modules/Old_Modules/Grand_Loops.tex <==
%%%% Currently not in use, as not needed. The math here seems correct, and could be useful in future(?)


\section{Grand Loops}

\textcolor{red}{In this section, we define the grand loops graph, and prove that it is quasi-isometric to the grand arc graph.}

\begin{defn}
    Let $\Sigma$ be an infinite-type surface.
    A \textit{loop} in $\Sigma$ is a simple arc with both endpoints converging to the same end.

    A loop $l$ is called \textit{grand} if it satisfies the following conditions:
    \begin{enumerate}
        \item Both endpoints of $l$ are maximal
        \item $l$ is separating
        \item Both connected components of $\Sigma \backslash l$ contain a grand arc.
    \end{enumerate}
\end{defn}

\begin{rmk}
    The third condition above is equivalent to there being  a maximal end in each connected component of $\Sigma\backslash l$.
\end{rmk}

\begin{lem}
    A loop is grand if and only if it is witness filling
\end{lem}

\begin{proof}
    TODO
    \textcolor{red}{ABN: I strongly suspect that this is true. One direction is easy: if the
    loop is grand, and not witness-filling, then there must be a witness
    contained in one connected component of $\Sigma \ssm l$, but then $l$ could
    not contain a grand arc in the other component. 
    }
\end{proof}

\begin{defn}
    The \textit{grand loop graph} $L(\Sigma)$, is the graph whose vertices are
    homotopy classes of grand loops, with edges between loops when they can be
    realized disjointly.
\end{defn}

The rest of this section is dedicated to proving the following lemma:

\begin{lem}
    $\calG(\Sigma)$ and $L(\Sigma)$ are quasi-isometric.
\end{lem}

To prove that these graphs are quasi-isometric, we construct two coarsely-defined Lipschitz maps, 
$f:L(\Sigma) \to \calG(\Sigma)$ and $g:\calG(\Sigma) \to L(\Sigma)$ as follows:
$$
    f(l) = \{\alpha \in \calG(\Sigma): |\alpha\cap l| = 0\}\\
    g(\alpha) = \{l \in L(\Sigma): |l\cap \alpha| = 0\}
$$

\begin{claim}
    $f$ and $g$ are coarsely well-defined. That is, for any $l \in L(\Sigma)$ 
    and $\alpha \in \calG(\Sigma)$, $\mathrm{diam}(f(l))$ 
    and $\mathrm{diam}(g(\alpha))$ are bounded uniformly.
\end{claim}

\begin{proof}
    We start by showing that $\mathrm{diam}(f(l)) \le 3$. Let $\alpha,\beta$ be
    grand arcs disjoint from $l$. If $\alpha$ and $\beta$ lie in distinct
    connect components of $\Sigma \ssm l$, then they must be disjoint. If 
    they lie in the same component, then any grand arc in the other component 
    must be disjoint from both. Thus, $d_{\calG(\Sigma)}(\alpha,\beta) \le 3$.

    Next, we show that $\mathrm{diam}(g(\alpha)
    
    

Claim:
For any $l$, $f(l)$ has diameter at most $2$.

Proof: Let $\Sigma_1,\Sigma_2$ be the connected components of $\Sigma \setminus l$, and let $\alpha,\beta$ be grand arcs disjoint from $l$. Up to replacing $\alpha$ with $\alpha' \in f(l)$ disjoint from $\alpha$, we can assume WLOG that $\alpha,\beta \subset \Sigma_1$. For any grand arc $\gamma \subset \Sigma_2$, we have $\alpha - \gamma -\beta$, and we're done.

Claim:

Suppose that $\Sigma$ has at least four maximal end types.
If $l_1,l_2$ are disjoint grand loops, then $f(l_1)$ and $f(l_2)$ intersect.

Proof: Let $\Sigma_1,\Sigma_2$ be the conn comp. comp. of $l_1$, WLOG $l_2$ is contained in $\Sigma_2$, and separates $\Sigma_3$ from a part of $\Sigma_2$. Any grand arc contained in $\Sigma_3$ will do.

**Notation**
$e(l)$ is the end that $l$ converges to.

Claim:

Suppose that $\Sigma$ has exactly three max end types, then $f(l_1)$ and $f(l_2)$ are close.

If $l_1$ and $l_2$ are disjoint, see above. Suppose $e(l_1)$ and  $e(l_2)$ are in distinct equivalence classes. Let $U(l_1,l_2)$ be the set of all unicorns between $l_1$ and $l_2$. 

Note that $|U(l_1,l_2)| \le 4$, and $U(l_1,l_2)$ consists of grand arcs. This means that there exists a sequence $x_1,...,x_n$ (with $n < 5$) such that $l_1 - x_1 - x_2 - x_3 - .. - x_n - l_2$ where  ( - ) means disjointness. In particular, $x_1 \in f(l_1)$ and $x_n \in f(l_2)$. So these sets are close.

If $e(l_1)$ and $e(l_2)$ are in the same equivalence class then pick maximal $e \in E(\Sigma)$ not equivalent to $e(l_i)$. Pick a path $\gamma$ from $e$ to $l_1$ which does not intersect $l_2$. $\gamma$ intersects $l_1$ at $p$, and the unicorn $x = \gamma *_p l_1$ is a grand arc disjoint from $l_1$, and which intersects $l_2$ at most twice.

Let $q$ be the first intersection of $x$ with $l_2$, since $|x \cap l_2| \le 2$, there exists a direction along $l_2$ for which $x_1 = x *_q l_2$ is simple and disjoint from $l_2$, and intersects $x$ at most once. Now, the standard "sidestep unicorn" argument for grand arcs will work between $x$ and $x_1$, so $d_G(x,x_1) < 4$,

$$
l_1 - x - \cdots - x_1 - l_2
$$

**In fact**:
We can use some combinatorics to show that regardless of the number of maximal ends ($\ge 3$), $f(l_1)$ and $f(l_2)$ intersect. 

Proof idea: 
Look at the intersections of the surfaces that $l_1$ and $l_2$ separate, and find a grand arc between them (uses a very strict constraint on the number of complementary components of $\Sigma \smallsetminus (l_1 \cup l_2))$.

---

**Define**
$g: G \to L$ sending $\alpha \to \{l : |l\cap \alpha| = 0\}$.

Claim:
For any $\alpha$, $g(\alpha)$ has finite diameter.

Proof:

Let $c$ be a simple closed curve int
**Proof missing**


Claim:

If $\alpha \sim \beta$ then $g(\alpha)$ and $g(\beta)$ are close.

Proof:

If there exists an end of $\beta$ which is not an end of $\alpha$, (use FGM + Grand arcs paper) choose $c$ to be a simple closed curve disjoint from $\alpha$, intersecting $\beta$ exactly once, and separating an end of $\beta$ from the rest of the ends of $\alpha$. Then $\beta * c * \beta$ is a grand loop disjoint from both $\alpha$ and $\beta$. 

If $e(\alpha) = e(\beta)$, find $\gamma$ disjoint from $\alpha$ and $\beta$ with different ends, and then $g(\alpha)$ intersects $g(\gamma)$ which intersects $g(\beta)$.




    


==> Modules/Old_Modules/Grand_rays.tex <==
Next, we shall show that if $m$ is a geodesic asymptotic to $L$ in $\Sigma$ (i.e. $m$ is a grand ray), then the bicorns with $m$ are also close to the bicorns with $L$.

\begin{defn}
Let $L\in\mathcal{GEL}\left(\Sigma\right)$ which fills a witness $W\subset\Sigma$. A geodesic $m\in\Gamma\left(\Sigma\right)$ to be a \emph{grand ray converging to $L$} if: 
\begin{enumerate}
\item $m$ converges to a maximal end of $\Sigma$, an open neighbourhood of which is disjoint from $W$, and
\item $m$ converges to $L$ asymptotically.
\end{enumerate}
\end{defn}

\begin{rmk}
    \textcolor{red}{Proof needed! Possibly refer to appendix.} Suppose $\Sigma$ is the once-punctured Cantor tree. Note that the ray graph of $\Sigma$ (as defined in \cite{B-W}) corresponds to $\mathcal{G}(\Sigma)$. Let $L\in \mathcal{GEL}(\Sigma)$. Then the collection of grand rays converging to $L$ corresponds to a clique of ``high-filling rays'' (Definition 2.7.1 in \cite{B-W}).  
\end{rmk}

For an example of a grand ray, see Figure \ref{fig:bicorns_with_asymptotic}.

\begin{lem}\label{lem:bicorns_with_grand_ray}
Let $L$ a minimal lamination on $\Sigma$ that fills a subsurface $S$ (not necessarily a witness), and $a\in\mathcal{G}\left(\Sigma\right)$. Let $m$ be a grand ray converging to $L$ and disjoint from $a$ outside $S$. Then as subsets of $\mathcal{G}\left(\Sigma\right)$, we have 
\[
d_{\mathrm{Haus}}\left(\mathcal{B}\left(a,m\right),\mathcal{B}\left(a,L\right)\right)\leq1.
\]
\end{lem}

\begin{proof}
Note that $\#m\cap\partial S=1$. If $a$ is disjoint from $S$, then the result is trivially true, so assume otherwise. Let $P$ be the first point of $a\cap m$ along $m$, oriented away from the maximal end it converges to (note that this exists, since $a\cap m$ is discrete and contained inside $S$). Since $L$ fills $S$, $a\cap L$ is not empty, and since $L$ is closed, there is a first point $Q$ of $a\cap L$ along $a$ traveling away from $P$ (in some orientation along $a$). Suppose $Q$ is on a leaf $l$. Consider unit-speed parametrizations on $l$ and $m$ with $m(0)=P$ and $l(0)=Q$. Then as parametrized geodesics, since $m$ is asymptotic to $L$, we get $d\left(m(t),l(t)\right)\to0$ as $t\to\infty$ (the choice of leaf $l$ here doesn't matter, since $L$ is minimal). So, every point of $a\cap m$ corresponds to a point of $a\cap l$, as shown in Figure \ref{fig:bicorns_with_asymptotic}.

\begin{figure}[h]
    \centering
    \includegraphics[width=10 cm, height=12 cm, keepaspectratio]{Pictures/bicorns_with_asymptotic.png}
    \caption{As $m$ is asymptotic to $L$, it bounds a rectangular region with $l$ and segments of $a$.}
    \label{fig:bicorns_with_asymptotic}
\end{figure}

Let $b=a_{1}\cup m_{1}\cup a_{2}$ be a bicorn in $\mathcal{B}\left(a,m\right)$, with $m_{1}\equiv\left(XY\right)_{m}$. Let $X',Y'$ be the points on $l$ corresponding to $X,Y$ respectively. Then $\left(X'Y'\right)_{l}$ defines a bicorn arc $b'\in\mathcal{B}\left(a,l\right)$ disjoint from $m$. Similarly, if $u=a_{3}\cup m_{2}$ is a unicorn arc in $\mathcal{B}\left(a,m\right)$ with $a_{3}\cap m_{2}=Z$. Then there are only finitely many points of $a\cap m_{2}$; let $Z'$ be the last point of $a\cap m_{2}$ along $a$ oriented along $a_{3}$ (if there are no such points, then $Z'=Z$). Then $\left(ZZ'\right)_{m}$ defines a bicorn arc $u'\in\mathcal{B}\left(a,l\right)$ disjoint from $u$. So, as subsets of $\mathcal{G}\left(\Sigma\right)$, we have $\mathcal{B}\left(a,m\right)\subset N_{1}\left(\mathcal{B}\left(a,l\right)\right)$. See Figure \ref{fig:unicorns_and_bicorns_asymptotic}.

\begin{figure}[h]
    \centering
    \includegraphics[width=12 cm, height=12 cm, keepaspectratio]{Pictures/unicorns_and_bicorns_asymptotic.png}
    \caption{We construct bicorns in $\mathcal{B}(a,l)$ disjoint from unicorns or bicorns in $\mathcal{B}(a,m)$.}
    \label{fig:unicorns_and_bicorns_asymptotic}
\end{figure}

Similarly, let $b=a_{1}\cup l_{1}\cup a_{2}$ be a bicorn in $\mathcal{B}\left(a,l\right)$. Since $m$ is asymptotic to $L$ and $l$ is dense in $L$, we can find a segment $m_{1}$ arbitrarily close to $l_{1}$ such that $m_{1}$ and $l_{1}$ bound an embedded rectangular region in $\Sigma$ with $a$. Then $m_{1}$ defines a bicorn in $\mathcal{B}\left(a,m\right)$ disjoint from $l$. It follows that $d_{\mathrm{Haus}}\left(\mathcal{B}\left(a,m\right),\mathcal{B}\left(a,L\right)\right)\leq1$.
\end{proof}

\begin{prop} \label{prop:unicorns_geodesic_conv}
Let $a\in\mathcal{G}\left(\Sigma\right)$ and $L$ a minimal lamination on $\Sigma$. Suppose that $L$ fills the subsurface $W$ (not necessarily a witness), and assume that $a$ intersects $W$ transversely. Suppose that some maximal end $e\in\mathrm{ends}(a)\backslash\mathrm{ends}(W)$. Let $m$ be a grand ray that agrees with $a$ in an open neighbourhood of $e$, is disjoint from $m$ outside $W$, and is asymptotic to $L$ in $W$. Then there exists a sequence $\left\{ b_{n}\right\} _{n\in\mathbb{N}}\subset\mathcal{B}\left(a,m\right)$ such that $b_{n}\to m$ in $\Gamma\left(\Sigma\right)$. 
\end{prop}


\begin{proof}
Similar to proof of Proposition \ref{prop:bicorns_geodesic_conv}, $a\cap m$ is an infinite discrete subset of $m$, and we can find an $\epsilon>0$ such that any two points of $a\cap m$ are at least distance $2\epsilon$ apart along $m$. What's different from the proof of Proposition \ref{prop:bicorns_geodesic_conv} is that $a\cap m$ will have a first point of intersection along $m$ (since $m$ is an isolated leaf in $m\cup L$, and agrees with $a$ in a neighbourhood of their common maximal end). 

Orient $a,m$ away from the end they converge to, and let $P_{0},P_{1},P_{2},\dots$ denote the points of $a\cap m$ as they appear along $m$. Note that any unicorn arc between $a$ and $m$ would be of the form $u=\left(\dots P_{i}\right)_{m}\cup\left(P_{i}\dots\right)_{a}$ (i.e. starts along $m$, ends along $a$). We shall construct a sequence of unicorn arcs $u_{i}=m_{i}\cup a_{i}$ with $m_{i}=\left(\dots P_{n_{i}}\right)_{m}$ and $a_{i}=\left(P_{n_{i}}\dots\right)_{a}$, with $n_{i}\to\infty$. We shall then show (similar to the proof of Proposition \ref{prop:bicorns_geodesic_conv}) that this sequence indeed converges to $m$ in $\Gamma\left(\Sigma\right)$.

Note that $P_{0}$ defines a unicorn arc $u_{0}=\left(\dots P_{0}\right)_{m}\cup\left(P_{0}\dots\right)_{a}$, so we inductively assume that $u_{i}=\left(\dots P_{n_{i}}\right)_{m}\cup\left(P_{n_{i}}\dots\right)_{a}$ is well defined. Set $P_{n_{i+1}}$ to be the first point of $u_{i}\cap m$ along $m$. Then $P_{n_{i+1}}$ defines a unicorn arc $u_{i+1}=\left(\dots P_{n_{i+1}}\right)_{m}\cup\left(P_{n_{i+1}}\dots\right)_{a}$ - indeed, $\left(P_{n_{i+1}}\dots\right)_{a}\subset a_{i}$, so $u_{i+1}$ is simple and disjoint from $u_{i}$. Moreover, $n_{i+1}>n_{i}$, so we indeed have $\left\{ n_{i}\right\} _{i\in\mathbb{N}}\to\infty$. See Figure \ref{fig:unicorns_converging_geodesically}.

\begin{figure}[h]
    \centering
    \includegraphics[width=12 cm, height=12 cm, keepaspectratio]{Pictures/unicorns_converging_geodesically.png}
    \caption{Inductively constructing the unicorn arc $u_{i+1}$ inductively from $u_{i}$. Note that unlike the bicorn sequence constructed in Proposition \ref{prop:bicorns_geodesic_conv}, $u_{i+1}$ is actually disjoint from $u_i$.}
    \label{fig:unicorns_converging_geodesically}
\end{figure}

Finally, choose a lift $\tilde{m}$ of $m$ to the universal cover $\mathbb{H}^{2}$, so that every point $P_{i}$ of $a\cap m$ corresponds to a lift $\tilde{a}_{i}$ of $a$ to $\mathbb{H}^{2}$. Once again, a necessary condition for the lifts $\tilde{u}_{i}$ of $u_{i}$ corresponding to $\tilde{m}$ to not converge to $\tilde{m}$ in $\Gamma\left(\mathbb{H}^{2}\right)$ is that the angle of intersection of $\tilde{a}_{i}$ and $\tilde{m}$ must go to $0$. But since $m$ converges to $L$ asymptotically, the angle of intersection of $a$ with $m$ is eventually close to the angle of intersection of $a$ with $l$, for any leaf $l\in L$. Thus, if angles of $a\cap m$ converged to $0$ along $m$, then so would the angles of intersection of $a\cap l$. This contradicts what we observed in the final paragraph in the proof of Proposition \ref{prop:bicorns_geodesic_conv}. Thus, the sequence $\left\{ u_{i}\right\} _{i\in\mathbb{N}}\subset\mathcal{B}\left(a,m\right)$ indeed converges to $m$ in $\Gamma\left(\Sigma\right)$.
\end{proof}


(The proof that you can construct a coarse-converging sequence of bicorns.)

==> Modules/Old_Modules/_old__Background.tex <==
This section should have a bunch of things - info about grand splittings, defn and results about grand arcs from Assaf-Yvon's work, stuff about minimal laminations (similar to Pho-On's chapter 2).

\textcolor{red}{Add lemma - Suppose there is a witness $W$ with a boundary component $\gamma$. Suppose $a,b$ be two grand arcs that intersect $\gamma$ exactly once, and all points of $a\cap b$ are in the component of $\Sigma - W$ corresponding to $\gamma$. Then $d_{\mathcal{G}}(a,b)\leq 2$.}

\begin{lem}
    Suppose $e_1,e_2$ are two ends of $\Sigma$ that are both maximal and not equivalent. Let $a\in \mathcal{G}(\Sigma)$. Then there is a grand arc $a'$ converging to $e_1$ and $e_2$ respectively, with $d_{\mathcal{G}}\left(a,a'\right)\leq 1$.
\end{lem}

\begin{lem}
Let $a,b\in\mathcal{G}\left(\Sigma\right)$. Suppose $a$ converges to the ends $e_{1},e_{2}$. Then there exists a grand arc $c$ which agrees with $a$ in an open neighbourhood of $e_{1},e_{2}$, and $d_{\mathcal{G}}\left(a,c\right)\leq3$ (if $\Sigma$ has at least four maximal end types, then this bound is actually $2$). 
\end{lem} 

==> Modules/Old_Modules/_old__Geodesic_Convergence.tex <==
\section{Geodesic Convergence}

Fix a \textit{Nielsen-convex} (see \cite{Tap}) hyperbolic metric on $\Sigma$, and fix a covering map $\pi\colon\mathbb{H}^{2}\to\Sigma$ corresponding to this metric. Let $\Gamma\left(\mathbb{H}^{2}\right)$ denote the space of geodesics in $\mathbb{H}^{2}$, equipped with the usual topology (this is homeomorphic to an open Möbius band). Let $\Gamma\left(\Sigma\right)$ denote the space of simple geodesics on $\Sigma$. Denote by $\Gamma_{\text{grand}}\left(\Sigma\right)$ the space of grand arcs on $\Sigma$ (note the distinction from $\mathcal{G}\left(\Sigma\right)$, which is the grand arc graph.)

\begin{defn}
We say that a sequence $\left\{ \lambda_{n}\right\} _{n\in\mathbb{N}}\subset\Gamma\left(\Sigma\right)$ \emph{geodesically converges} to $\lambda\in\Gamma\left(\Sigma\right)$ if there exist unit-speed parametrisations for each $\lambda_{n}$ and for $\lambda$, such that for every $\epsilon>0$ small and every $R>0$ large, there exists $N\in\mathbb{N}$ such that $d_{\Sigma}\left(\lambda_{n}(t),\lambda(t)\right)<\epsilon$ for every $n\geq N$ and for each $t\in\left[-R,R\right]$. 
\end{defn}

Note that a sequence $\left\{ \lambda_{n}\right\} _{n\in\mathbb{N}}$ may geodesically converge to multiple different geodesics in $\Gamma\left(\Sigma\right)$, based on the choice of parametrisations (for example, consider the Dehn twist sequence). That is to say, the space $\Gamma\left(\Sigma\right)$ with the topology of geodesic convergence is not Hausdorff.

\begin{lem} \label{lem:simple_closed}
The subspace $\tilde{\Gamma}\left(\Sigma\right)=\left\{ \gamma\in\Gamma\left(\mathbb{H}^{2}\right)\mid\pi\left(\gamma\right)\text{ is simple}\right\} $ is a closed subspace of $\Gamma\left(\mathbb{H}^{2}\right)$. 
\end{lem}

\begin{proof}
Restated, suppose $\left\{ \gamma_{n}\right\} _{n\in\mathbb{N}}$ is a sequence in $\Gamma\left(\mathbb{H}^{2}\right)$ which converge to a geodesic $\gamma_{0}$, and suppose that $\pi\left(\gamma_{i}\right)$ is simple for each $i$. We want to show that $\pi\left(\gamma_{0}\right)$ is simple. If not, then there is some point of self-intersection of $\pi\left(\gamma_{0}\right)$ - say a point $p\in\Sigma$, having lifts $\tilde{p}_{1}$ and $\tilde{p}_{2}$ on $\gamma_{0}$. Then by cover-convergence, for $n$ large enough, we must have self-intersection on $\pi\left(\gamma_{n}\right)$, contradicting that $\pi\left(\gamma_{i}\right)$'s were all simple.
\end{proof}




\ignore{
\begin{lem}\label{lem:geod_cover_convg}
A sequence $\left\{ \lambda_{n}\right\} _{n\in\mathbb{N}}\subset\Gamma\left(\Sigma\right)$ geodesically converges to $\lambda\in\Gamma\left(\Sigma\right)$ if and only if for every lift $\tilde{\lambda}$ of $\lambda$, we can choose a sequence of lifts $\tilde{\lambda}_{n}$ of $\lambda_{n}$ such that $\tilde{\lambda}_{n}\to\tilde{\lambda}$ in $\Gamma\left(\mathbb{H}^{2}\right)$.
\end{lem}

\begin{proof}
First, suppose we have a sequence $\left\{ \lambda_{n}\right\}
_{n\in\mathbb{N}}$ of simple geodesics on $\Sigma$ that geodesically converges to a geodesic
$\lambda$. Then as we can parametrise the geodesics such that for any $R>0$, we have that the
segments $\left\{ \lambda_{n}\left(\left[-R,R\right]\right)\right\}
_{n\in\mathbb{N}}$ Hausdorff-converge to $\lambda\left(\left[-R,R\right]\right)$
on $\Sigma$. Now, if $p,q\in\Sigma$ and $d_{\Sigma}\left(p,q\right)<\epsilon$ for some $\epsilon>0$, then for any lift $\tilde{p}$ of $p$, there is a lift $\tilde{q}$ of $q$ such that $d_{\mathbb{H}^{2}}\left(\tilde{p},\tilde{q}\right)<\epsilon$. Thus, for any lift $\tilde{\lambda}$ of $\lambda$, there are lifts $\tilde{\lambda}_{i}$ of $\lambda_{i}$ such that the segments $\tilde{\lambda}_{i}\left(\left[-R,R\right]\right)$ Hausdorff-converge to $\tilde{\lambda}\left(\left[-R,R\right]\right)$. Since this is true for every $R>0$, it follows that $\left\{ \tilde{\lambda}_{i}\right\} $ converges to $\tilde{\lambda}$ in $\Gamma\left(\mathbb{H}^{2}\right)$. 


Conversely, suppose we have a sequence $\left\{ \mu_{n}\right\}
_{n\in\mathbb{N}}$ in $\Gamma\left(\Sigma\right)$ and a simple geodesic $\mu$ on $\Sigma$ such that for any lift $\tilde{\mu}$ of $\mu$, we can choose a sequence $\tilde{\mu}_n$ of lifts of $\mu_n$ which converges to $\tilde{\mu}$ in $\Gamma(\mathbb H^2)$. Pick any point $p$ on $\tilde{\mu}$, and parametrize $\tilde{\mu}$ with unit
speed. Converges in $\Gamma(\mathbb H^2)$ implies that for any
$\epsilon,R>0$, we can find $N\in\mathbb{N}$ such that 
\[
d_{\mathbb{H}^{2}}\left(\tilde{\mu}_{n}(t),\tilde{\mu}(t)\right)<\epsilon
\]
for any $n\geq N$ and $t\in\left[-R,R\right]$. Since 
\[
d_{\Sigma}\left(\mu_{n}(t),\mu(t)\right)\leq d_{\mathbb{H}^{2}}\left(\tilde{\mu}_{n}(t),\tilde{\mu}(t)\right),
\]
the conclusion follows.
\end{proof}
}




\begin{lem}
Suppose a sequence $\left\{ \lambda_{n}\right\} _{n\in\mathbb{N}}\subset\Gamma\left(\Sigma\right)$ geodesically converges to distinct geodesics $\mu,\eta\in\Gamma\left(\Sigma\right)$. Then $\mu$ and $\eta$ are disjoint.
\end{lem}

\begin{proof}
Suppose $\mu$ and $\eta$  intersect transversely at some point $p$. Parametrise each  $\lambda_{i}$ and $\mu$ so that $\lambda_{i}\to\mu$ geodesically. Since these are unit-speed parametrisations, we could pick $\mu(0)=p$, and this would only cause the parametrisations to shift by a constant. In other words, there is a $T_{\mu}\in\mathbb{R}$ such that for every $\epsilon>0$ and $R>0$, there exists an $N\in\mathbb{N}$ large enough so that $d_{\Sigma}\left(\lambda_{n}\left(t+T_{\mu}\right),\mu(t)\right)<\epsilon$ for every $n\geq N$ and each $t\in\left[-R,R\right]$ (in fact, this $\mu(T_{\mu})=p$ in the original parametrisation). Similarly, we can find $T_{\eta}\in\mathbb{R}$ corresponding to $\eta$, and reparametrise $\eta$ so that $\eta(0)=p$.

Thus, we can choose $\epsilon>0$ small enough so that the $\epsilon$-neighbourhood of $p$ is an embedded disk, and $R>>2\epsilon$. Then for $n$ large enough, $\mu(0)=\eta(0)$ implies that $\lambda_{n}\left(t\right)=\lambda_{n}\left(t'\right)$ for some $t,t'\in\mathbb{R}$, contradicting that $\lambda_{n}$ is simple.
\end{proof}

%\textcolor{red}{Ignore the rest of this section - it is being rewritten below.}

%\subsection{Grand Laminations}


%\begin{lem}\label{lem:grand_lams_witness_filling}
%Every $\Lambda\in\tilde{\Gamma}_{\mathrm{grand}}\left(\Sigma\right)$ intersects every witness transversely. 
%\end{lem}

%\begin{proof}
%Let $\Lambda$ be a grand lamination corresponding to the limit set of $\left\{ x_{n}\right\} _{n\in\mathbb{N}}\subset\Gamma_{\mathrm{grand}}\left(\Sigma\right)$, and let $W$ be a witness. Every grand arc must intersect $W$ transversely (in fact, every grand arc must intersect at least two distinct components of $\partial W$). Let $\Gamma\left(W\right)$ be the subset of $\Gamma\left(\Sigma\right)$ of geodesics intersecting $W$ transversely. We shall show that $\Gamma(W)$ is a compact subset of $\Gamma\left(\Sigma\right)$. To see this, pick a fundamental domain for $\Sigma$ in $\mathbb{H}^{2}$, and fix a polygon $\tilde{W}$ which is the lift of $W$ contained in this fundamental domain. The collection of geodesics intersecting $\tilde{W}$ is a compact subspace of $\Gamma\left(\mathbb{H}^{2}\right)$. The subspace of these whose projections are simple is a closed subspace by Lemma \ref{lem:simple_closed}, and hence compact. Since, $\Gamma\left(W\right)$ is a quotient of a compact space  by the covering map, it is compact. 

%Thus, we can find a subsequence $\left\{ x_{n_{i}}\right\} _{i\in\mathbb{N}}$ of $\left\{ x_{n}\right\} _{n\in\mathbb{N}}$ which converges to a geodesic $\lambda\in\Gamma(W)\subset\Gamma\left(\Sigma\right)$. Since $\Lambda$ is the full limit set of $\left\{ x_{n}\right\} _{n\in\mathbb{N}}$, we must have $\lambda\in\Lambda$. In particular, $\Lambda$ intersects $W$.
%\end{proof}

%Note - each individual leaf of a grand lamination may be disjoint from some witness (eg. Dehn twisting) but the union of the leaves must intersect every witness.

%\begin{defn}
%Let $\left\{ x_{n}\right\} _{n\in\mathbb{N}}\subset\Gamma_{\mathrm{grand}}\left(\Sigma\right)$ and $\Lambda\in\tilde{\Gamma}_{\mathrm{grand}}\left(\Sigma\right)$. We say that $\left\{ x_{n}\right\} _{n\in\mathbb{N}}$ \emph{geodesically converges} to $\Lambda$ if $\Lambda$ is the full limit set under geodesic convergence of $\left\{ x_{n}\right\} _{n\in\mathbb{N}}$. 
%\end{defn}

%We next prove that the space of grand laminations with the topology of geodesic convergence is sequentially compact.

%\begin{prop}\label{prop:grand_laminations_compact}
%Let $\left\{ x_{n}\right\} _{n\in\mathbb{N}}\subset\Gamma_{\mathrm{grand}}\left(\Sigma\right)$.  There exists a subsequence $\left\{ x_{n_{i}}\right\} _{i\in\mathbb{N}}$ of $\left\{ x_{n}\right\} _{n\in\mathbb{N}}$ such that $x_{n_{i}}\to\Lambda\in\tilde{\Gamma}_{\mathrm{grand}}\left(\Sigma\right)$. 
%\end{prop}

%\begin{proof}
%Consider a compact exhaustion of $\Sigma$ by witnesses $\left\{ W_{i}\right\} _{i\in\mathbb{N}}$ such that $W_{i}\subset W_{i+1}$ for all $i$, and $\cup_{i\in\mathbb{N}}W_{i}=\Sigma$. First note that for all $i$, since $W_i$ is compact, the set 
%\[
%\Gamma\left(W_{i}\right)=\left\{ \gamma\in\Gamma\left(\Sigma\right)\mid\gamma\text{ intersects }W_{i}\text{ transversely}\right\} 
%\]
%is a compact subspace of $\Gamma(\Sigma)$. \ignore{(as shown in the proof of Lemma \ref{lem:grand_lams_witness_filling})} Moreover, for any $i>j$, we have that $W_{i}\subset W_{j}$, so that $\Gamma\left(W_{i}\right)\subset\Gamma\left(W_{j}\right)$, and $\Gamma_{\mathrm{grand}}\left(\Sigma\right)\subset\Gamma\left(W_{0}\right)$. 




%Thus, we have a sequence $\left\{ x_{n}^{0}\right\} _{n\in\mathbb{N}}\subset\left\{ x_{n}\right\} _{n\in\mathbb{N}}$ such that each $x_{i}^{0}\in\Gamma\left(W_{0}\right)$, and there exists $\lambda_{0}\in\Gamma\left(W_{0}\right)$ such that $\left\{ x_{n}^{0}\right\} \to\lambda_{0}$ geodesically. Let $\Lambda_{0}\subset\Gamma\left(W_{0}\right)$ be the collection of all such limits, i.e., 
%\[
%\Lambda_{0}=\left\{ \lambda_{0}\in\Gamma\left(W_{0}\right)\mid\left\{ x_{n}^{0}\right\} \to\lambda_{0}\right\} .
%\]
%Note that this is not yet a grand lamination, since we are taking the full limit set in $\Gamma\left(W_{0}\right)$, not $\Gamma\left(\Sigma\right)$. Inductively, for each $i\geq1$, we can find a subsequence $\left\{ x_{n}^{i}\right\} \subset\left\{ x_{n}^{i-1}\right\} $ which converges in $\Gamma\left(W_{i}\right)$, and define $\Lambda_{i}\subset\Gamma\left(W_{i}\right)$ to be the geodesic convergence limit of $\left\{ x_{n}^{i}\right\} $. Note that $\Lambda_{i}\subset\Lambda_{i+1}$, where in each instance we add the geodesics that intersect $W_{i+1}$ but not $W_{i}$. 

%Consider the diagonal sequence $\left\{ x_{n}^{n}\right\} _{n\in\mathbb{N}}$. This geodesically converges in $\Gamma\left(W_{i}\right)$ for any $i\geq0$. Let $\Lambda=\cup_{i\geq0}\Lambda_{i}$, which is a collection of disjoint simple geodesics in $\Sigma$. Then for any $\lambda\in\Lambda$, we have $\lambda\in\Lambda_{i}$ for some $i\geq0$, and $x_{n}^{n}\to\lambda$ by construction. On the other hand, any $\mu\in\Gamma\left(\Sigma\right)$ must intersect some $W_{i}$ (since it is a compact exhaustion), so $\mu\in\Lambda_{i}$ (since it was the full limit set). This proves that $x_{n}^{n}\to\Lambda$, as desired. 
%\end{proof} 

\ignore{

\begin{lem} \label{lem:disjt_convergence}
Suppose $\left\{ x_{n}\right\} _{n\in\mathbb{N}},\left\{ y_{n}\right\} _{n\in\mathbb{N}}\subset\Gamma_{\mathrm{grand}}\left(\Sigma\right)$ such that there are $\Lambda,\Lambda'\in\tilde{\Gamma}_{\mathrm{grand}}\left(\Sigma\right)$ with $x_{n}\to\Lambda$ and $y_{n}\to\Lambda'$. If $x_{n}\cap y_{n}=\emptyset$ for every $n\in\mathbb{N}$, then $\Lambda,\Lambda'$ are also disjoint, i.e., every leaf of $\Lambda$ is disjoint from every leaf of $\Lambda'$. 
\end{lem}

\begin{proof}
Suppose for contradiction that there are leaves $\lambda\in\Lambda$ and $\lambda'\in\Lambda'$  that intersect at a point $P$. Parametrize $\lambda$ and $\lambda'$ setting $\lambda(0)=\lambda'(0)=P$. Consider a lift $\tilde{P}$ of $P$ to $\mathbb{H}^{2}$, and consider the corresponding lifts $\tilde{\lambda}$ and $\tilde{\lambda'}$ of $\lambda$ and $\lambda'$. By Lemma \ref{lem:geod_cover_convg}, we have a sequence of lifts $\tilde{x}_{n}$ of $x_{n}$ and $\tilde{y}_{n}$ of $y_{n}$ that converge to $\tilde{\lambda}$ and $\tilde{\lambda'}$ respectively. Then for $n$ large enough, we must have that $\tilde{x}_{n}$ intersects $\tilde{y}_{n}$, which contradicts that $x_{n}$ and $y_{n}$ are disjoint.
\end{proof}


\ignore{
\begin{lem}
Suppose $\left\{ x_{n}\right\} _{n\in\mathbb{N}},\left\{ y_{n}\right\} _{n\in\mathbb{N}}\subset\Gamma_{\mathrm{grand}}\left(\Sigma\right)$ and suppose there exists $\Lambda\in\tilde{\Gamma}_{\mathrm{grand}}\left(\Sigma\right)$ such that $x_{n}\to\Lambda$ and $y_{n}\to\Lambda$. Then there exists $C>0$ such that 
\[
d_{\mathrm{Haus}}\left(\left\{ x_{n}\right\} _{n\in\mathbb{N}},\left\{ y_{n}\right\} _{n\in\mathbb{N}}\right)<C.
\]

Notes - specify dHaus in graph not surface.

\end{lem}


\abn{Under the assumptions that $\{x_n\}$ and $\{y_n\}$ are quasi-geodesic paths in the grand arc graph that start at the same point, it's enough to show that for sufficiently large $n$, $d_{\mathcal{G}(\Sigma)}(x_n, y_n)$ is controlled.}

\begin{proof}
Since $\left\{ x_{n}\right\} _{n\in\mathbb{N}}$ and $\left\{ y_{n}\right\} _{n\in\mathbb{N}}$ both geodesically converge to $\Lambda$, we can parametrize the grand arcs so that for any $\epsilon>0$ and any $R>0$, there exists $N\in\mathbb{N}$ such that for all $n\geq N$, 
\[
d_{\Sigma}\left(x_{n}(t),y_{n}(t)\right)<\epsilon
\]
for all $t\in\left[-R,R\right]$. Suppose the Hausdorff distance between $\left\{ x_{n}\right\} $ and $\left\{ y_{n}\right\} $ is unbounded. Then for any $C>0$, there exists a witness $W$ and $i,j\in\mathbb{N}$ such that $d_{W}\left(x_{i},y_{j}\right)>C$. 


\textcolor{red}{Proof incomplete}
\end{proof}


\textcolor{blue}{Question - Let $\gamma\in\Gamma\left(\Sigma\right)$ such that $\gamma$ does not converge to a non-maximal end. Then can we find a sequence $\left\{ x_{n}\right\} _{n\in\mathbb{N}}\in\Gamma_{\mathrm{grand}}\left(\Sigma\right)$ such that $x_{n}\to\gamma$? If yes, this means that every such geodesic is the leaf of some grand lamination.
}

} }


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%Topology of geodesic convergence.



Let $\gamma\in\Gamma\left(\Sigma\right)$ be parametrised. Then for any $R,\epsilon>0$, let 
\[
U_{R,\epsilon}\left(\gamma\right)=\left\{ \gamma'\in\Gamma\left(\Sigma\right)\text{ parametrised}\mid d_{\Sigma}\left(\gamma(t),\gamma'(t)\right)<\epsilon\text{ for all }t\in\left[-R,R\right]\right\} .
\]
Then $\left\{ U_{R,\epsilon}\left(\gamma\right)\right\} _{R,\epsilon>0}$ forms a neighbourhood basis for $\gamma$ with the topology of geodesic convergence. Moreover, it suffices to choose one of countably many unit-speed parametrisations for $\gamma$ by starting at $\gamma(n)$ for any $n\in\mathbb{Z}$ (where the initial chosen parametrisation is the one starting at $\gamma(0)$. Letting $R\in\mathbb{N}$ and $\epsilon=\frac{1}{n}$ for some $n\in\mathbb{N}$ is also sufficient, so $\Gamma(\Sigma)$ is first-countable with the topology of geodesic convergence. In particular, for any subspace of $\Gamma\left(\Sigma\right)$, compactness is equivalent to sequential compactness.


\begin{lem}
Let $K\subset\Sigma$ be compact. Let $\Gamma\left(K\right)$ denote the subspace of $\Gamma\left(\Sigma\right)$ consisting of geodesics in $\Sigma$ that transversely intersect $K$. Then $\Gamma(K)$ is compact.
\end{lem}

\begin{proof}
We wish to prove that for any sequence $\left\{ \gamma_{n}\right\} _{n\in\mathbb{N}}\subset\Gamma(K)$, there exists some $\gamma_{0}\in\Gamma(K)$ and a subsequence $\left\{ \gamma_{n_{k}}\right\} _{k\in\mathbb{N}}$ of $\left\{ \gamma_{n}\right\} _{n\in\mathbb{N}}$ such that $\gamma_{n_{k}}\to\gamma_{0}$ geodesically. Choose a compact exhaustion $K=K_{0}\subset K_{1}\subset\dots$ of $\Sigma$. For each $i\geq1$, let $\left\{ \gamma_{k}^{i}\right\} _{k\in\mathbb{N}}\subset\left\{ \gamma_{n}^{i-1}\right\} _{n\in\mathbb{N}}$ (where $\gamma_{n}^{0}\equiv\gamma_{n}$) such that $\left\{ \gamma_{k}^{i}\cap K_{i}\right\} _{k\in\mathbb{N}}$ Hausdorff-converges to a lamination $L_{i}\subset K_{i}$ (we can find such a subsequence, since the space of geodesic laminations in a compact surface is compact with the Hausdorff topology). Note further that by construction, $L_{i}\subset L_{j}$ for $i<j$, and each $L_{i}$ is non-empty since each $\gamma_{i}$ intersects each $K_{n}$.

Then, consider the diagonal sequence $\left\{ \gamma_{i}^{i}\right\} _{i\in\mathbb{N}}\subset\left\{ \gamma_{n}\right\} _{n\in\mathbb{N}}$. Let $\Lambda=\cup_{i\ge0}L_{i}$. We get that for any compact subsurface $V$ of $\Sigma$, $\left\{ \gamma_{i}^{i}\cap V\right\} _{i\in\mathbb{N}}$ Hausdorff-converges to the lamination $\Lambda\cap V$ in $V$ (simply by recognizing $V$ as a subsurface of some $L_{j}$). We claim that $\left\{ \gamma_{i}^{i}\right\} _{i\in\mathbb{N}}$ geodesically converges to every leaf of $\Lambda$. To see this, let $l\in\Lambda$, pick a parametrization on $l$, choose $R,\epsilon>0$, and consider $N_{\epsilon}\left(l\left(\left[-R,R\right]\right)\right)$. We can find $j>>0$ such that $N_{\epsilon}\left(l\left(\left[-R,R\right]\right)\right)\subset K_{j}$, so that $l\left(\left[-R,R\right]\right)\subset L_{j}$. Since $\left\{ \gamma_{i}^{i}\cap K_{j}\right\} _{i\in\mathbb{N}}$ Hausdorff-converges to $L_{j}$, we get that $\left\{ \gamma_{i}^{i}\right\} _{i\in\mathbb{N}}$ geodesically converges to $l$. 

Finally, since each $\gamma_{n}$ intersects $K$ transversely, so does $\Lambda$. So, we can pick $l\in\Lambda$ in the above paragraph to intersect $K$ transversely. The conclusion follows. 
\end{proof}

\begin{rem}
The above proof does not depend on the choice of $K$. We end up choosing a compact exhaustion for $\Sigma$ and building the limiting geodesic by diagonalization. However, it is important that all the $\gamma_{i}$'s intersect $K$ - for example, if we choose a sequence of simple closed curves contained in disjoint compact surfaces that limit to an end, then no subsequence of this sequence would geodesically converge.
\end{rem}

%
\begin{cor}
$\Gamma_{\mathrm{grand}}\left(\Sigma\right)$ is compact. 
\end{cor}


\begin{lem}
Let $\left\{ a_{n}\right\} _{n\in\mathbb{N}}$ be a sequence of grand arcs, and let $\lambda=\left\{ l\in\Gamma\left(\Sigma\right)\mid a_{n}\xrightarrow{\text{geodesic}}l\right\} .$ Then $\Lambda$ is closed as a subset of $\Gamma\left(\Sigma\right)$. 
\end{lem}

\begin{proof}
Suppose $l_{0}\in\Gamma\left(\Sigma\right)$ be a geodesic in the closure of $\lambda$; we shall prove that $\left\{ a_{n}\right\} _{n\in\mathbb{N}}$ geodesically converges to $l_{0}$. 

Pick a parametrization on $l_{0}$, and choose $R,\epsilon>0$. Consider the segment $l_{0}\left[-R,R\right]$. Since it is compact, and in the closure of $\lambda$, we can choose finitely many $l_{i}\in\lambda$ (for $i=1,2,\dots,k$), such that 
\[
l_{0}\left(\left[-R,R\right]\right)\subset\underset{i\leq k}{\cup}N_{\epsilon/2}\left(l_{i}\left(\left[-R,R\right]\right)\right).
\]
Since $\left\{ a_{n}\right\} _{n\in\mathbb{N}}$ geodesically converges to each $l_{i}$, there exists an $N_{i}$ such that for all $n\geq N_{i}$, 
\[
d_{\Sigma}\left(a_{n}(t),l_{i}(t)\right)<\frac{\epsilon}{2}
\]
for $t\in\left[-R,R\right]$. Let $N=\sup_{i\leq k}N_{i}$. Then by the triangle inequality, for all $n\geq N$, 
\[
d_{\Sigma}\left(a_{n}(t),l_{0}(t)\right)<\epsilon
\]
for all $t\in\left[-R,R\right]$, as desired.
\end{proof}

\begin{cor}
If $\left\{ a_{n}\right\} _{n\in\mathbb{N}}$ is a sequence of grand arcs, then the full limit set of $\left\{ a_{n}\right\} _{n\in\mathbb{N}}$ under geodesic convergence is a geodesic lamination on $\Sigma$.
\end{cor}

\textcolor{blue}{Note here about how cover convergence relates to geodesic convergence? Do we want one over the other?}


\begin{defn}
Let $\left\{ L_{n}\right\} _{n\in\mathbb{N}}$ be a sequence of geodesic laminations in $\Sigma$. We say that $\left\{ L_{n}\right\} _{n\in\mathbb{N}}$ \emph{coarse geodesically converges to }a lamination $L$, if for any subsequence $\left\{ L_{n_{k}}\right\} _{k\in\mathbb{N}}$ that geodesically converges to a lamination $L'$, we must have that $L\subset L'$. Equivalently, we say that a sequence of geodesics $\left\{ \gamma_{n}\right\} _{n\in\mathbb{N}}$ \emph{coarse-geodesically converges} to a lamination $L$ if for any subsequence $\left\{ \gamma_{n_{k}}\right\} _{k\in\mathbb{N}}$ that geodesically converges to some lamination $\Lambda$, we have $L\subset\Lambda$. 
\end{defn}



Motivating example for this definition - consider a simple closed curve $\gamma$ in $\Sigma$, and two disjoint grand arcs $a,b$ that both intersect $\gamma$. Let $a_{n}=T_{\gamma}^{n}\left(a\right)$ and $b_{n}=T_{\gamma}^{n}\left(b\right)$, and let 
\[
c_{n}=\begin{cases}
a_{n/2} & n\text{ even}\\
b_{\left(n+1\right)/2} & n\text{ odd}
\end{cases}.
\]
Then the full limit set of $c_{n}$ under geodesic convergence is just the curve $\gamma$, while the subsequences $\left\{ a_{n}\right\} _{n\in\mathbb{N}}$ and $\left\{ b_{n}\right\} _{n\in\mathbb{N}}$ each geodesically converge to $\gamma$ along with two isolated leaves that converge to the same ends as $a$ and $b$ respectively. Then $\left\{ c_{n}\right\} _{n\in\mathbb{N}}$ coarse geodesically converges to $L=\left\{ \gamma\right\} $, and so do $\left\{ a_{n}\right\} _{n\in\mathbb{N}}$ and $\left\{ b_{n}\right\} _{n\in\mathbb{N}}$. 

In particular, by definition, if a sequence coarse geodesically converges to a lamination, then so do all its subsequences.





%






==> Modules/Old_Modules/_old__Grand_laminations.tex <==
%%This is when we did grand laminations as full limitsets.

\section{Grand Laminations}

Notation - let $\mathcal{G}\left(\Sigma\right)$ denote the grand arc graph of $\Sigma$. Let $\Gamma_{\mathrm{grand}}\left(\Sigma\right)$ denote the space of grand arcs on $\Sigma$, with the topology of geodesic convergence. Note that $d_{\mathcal{G}}$ will refer to the graph distance between two grand arcs.  

\begin{defn}
A \emph{grand lamination} $\Lambda$ is a collection of pairwise disjoint elements in $\Gamma\left(\Sigma\right)$, which form the full limit set (under geodesic convergence) of some convergent sequence $\left\{ x_{i}\right\} _{i\in\mathbb{N}}$ of grand arcs. In other words, \[
\Lambda\left(x_n\right)=\left\{ \lambda\in\Gamma\left(\Sigma\right)\mid  x_{n}\to\lambda\text{ geodesically}\right\}.
\]
Denote the space of grand laminations on $\Sigma$ as $\tilde{\Gamma}_{\mathrm{grand}}\left(\Sigma\right)$, with the topology induced from $\Gamma\left(\Sigma\right)$. 

\end{defn}

Note that a single grand arc is a grand lamination. Given a finite collection of pairwise disjoint grand arcs, we can find a larger finite collection of pairwise disjoint grand arcs which is a grand lamination.

\begin{defn}
Let $\mathcal{GL}\left(\Sigma\right)$, the \emph{grand lamination graph}, be a graph whose vertices correspond to grand laminations. Two grand laminations $\Lambda$ and $\Lambda'$ are connected by an edge if their leaves are disjoint, and they can be realized by geodesically convergent sequences $\left\{ c_{n}\right\} _{n\in\mathbb{N}}$ and $\left\{ c_{n}'\right\} _{n\in\mathbb{N}}$ of grand arcs, such that $c_{n}\xrightarrow{\mathrm{geod}}\Lambda$ and $c_{n}'\xrightarrow{\mathrm{geod}}\Lambda'$, with $c_{n}\cap c_{n}'=\phi$ for all $n$. 
\end{defn}

This condition on edges is stronger than just disjointness, and necessarily so. For example, let $W$ be a compact witness in $\Sigma$, and let $V$ be a subsurface of $\Sigma$ which is contained in a component of $\Sigma\backslash W$. Pick $\lambda$ and $\mu$ to be some ending laminations on $W$ and $V$, respectively. Lemma \ref{lem:minimal_lam_grand} below shall prove that these are indeed grand laminations on $\Sigma$. Let $x$ be a grand arc disjoint from $\mu$ (which exists since $V$ is not a witness). We want to say that $\lambda$ corresponds to a point in $\partial\mathcal{G}\left(\Sigma\right)$, but not $\mu$. In particular, even though $\mu$ is disjoint from both $x$ and $\lambda$, 
\[
x-\mu-\lambda
\]
is NOT a path in $\mathcal{GL}\left(\Sigma\right)$, as the sequences of grand arcs that geodesically converge to $\mu$ and $\lambda$ cannot remain disjoint. 

On the other hand, note that $\mathcal{G}(\Sigma) \subset \mathcal{GL}(\Sigma)$ as graphs (i.e. disjoint grand arcs remain adjacent in $\mathcal{GL}(\Sigma)$.

\begin{lem}
Every grand lamination is closed.
\end{lem}

\begin{proof}
Let $\lambda$ be a grand lamination, which is the full limit set of a geodesically convergent sequence of grand arcs $\left\{ a_{n}\right\} _{n\in\mathbb{N}}$. Suppose $l_{0}\in\Gamma\left(\Sigma\right)$ be a geodesic in the closure of $\lambda$; we shall prove that $\left\{ a_{n}\right\} _{n\in\mathbb{N}}$ geodesically converges to $l_{0}$. 

Pick a parametrization on $l_{0}$, and choose $R,\epsilon>0$. Consider the segment $l_{0}\left[-R,R\right]$. Since it is compact, and in the closure of $\lambda$, we can choose finitely many leaves $l_{i}\in\lambda$ (for $i=1,2,\dots,k$), such that 
\[
l_{0}\left(\left[-R,R\right]\right)\subset\underset{i\leq k}{\cup}N_{\epsilon/2}\left(l_{i}\left(\left[-R,R\right]\right)\right).
\]
Since $\left\{ a_{n}\right\} _{n\in\mathbb{N}}$ geodesically converges to each $l_{i}$, there exists an $N_{i}$ such that for all $n\geq N_{i}$, 
\[
d_{\Sigma}\left(a_{n}(t),l_{i}(t)\right)<\frac{\epsilon}{2}
\]
for $t\in\left[-R,R\right]$. Let $N=\sup_{i\leq k}N_{i}$. Then by the triangle inequality, for all $n\geq N$, 
\[
d_{\Sigma}\left(a_{n}(t),l_{0}(t)\right)<\epsilon
\]
for all $t\in\left[-R,R\right]$, as desired.
\end{proof}


\begin{rem}
This means that geodesic convergence is weaker than cover convergence. For example, in the Dehn twist example, the grand lamination consists of the two leaves converging to the two ends as well as the simple closed curve. The sequence of grand arcs cover converges to both the leaves that go to ends, but only geodesically converges to the simple closed curve.
\end{rem}



\begin{lem}\label{lem:grand_unicorns_geod_conv}
Let $\lambda$ be a closed, minimal lamination which is not a single simple closed curve, and whose support is not all of $\Sigma$. Then there exists a grand lamination $\Lambda$ such that $\lambda\subset\Lambda$ and $\Lambda\backslash\lambda$ contains at most two isolated leaves.
\end{lem}

\begin{proof}
(Proof idea) By assumption, we can construct a geodesic arc $\gamma$ disjoint from $\lambda$, which converges to a maximal end on one side, and is asymptotic to (some leaf of) $\lambda$ along the other. Note that $\gamma$ is NOT a grand arc, as $u$ doesn't converge to any end on the other side.

Now, let $a$ be a grand arc that intersects $\lambda$, and which does not converge to the end that $\gamma$ converges to. In particular, consider $V=\overline{N_{\epsilon}\left(\lambda\right)}$. If there is some grand arc contained in $V$, then set this to be $a$. Else, choose a grand arc that intersects $\partial V$ minimally - i.e. a grand arc $a$ that intersects $\partial V$ once in at most two different components. Then we can define unicorn arcs (similar to Pho On) between $a$ and $\gamma$; call this path $\left\{ u_{n}\right\} _{n\in\mathbb{N}}$. These are well-defined, for any $t\in\mathbb{R}$, we must have that $\#a\cap\left(\gamma\mid_{\left(-\infty,t\right)}\right)<\infty$. 

By minimality, we can now copy the proof of Pho On's Lemma 3.2 to say that the unicorn path $\left\{ u_{n}\right\} _{n\in\mathbb{N}}$ geodesically converges to every leaf of $\lambda$. Moreover, the other leaves of $\Lambda$ correspond to parts of $a$ in $\Sigma-V$ (away from $\lambda$), which are constant across the $u_{n}$'s. So these converge to (at most two) isolated leaves.
\end{proof}


\begin{lem} \label{lem:minimal_lam_grand}
A closed, connected, minimal lamination $\lambda$ on $\Sigma$ is a grand lamination. That is, there exists a sequence of grand arcs $\left\{ a_{i}\right\} _{i\in\mathbb{N}}$ whose full limit set under geodesic convergence is $\lambda$. 
\end{lem}

\begin{proof}
If $\lambda$ is a single simple closed curve, consider two grand arcs $x$ and $y$ that are disjoint, and intersect $\lambda$. Let $T_{\lambda}$ denote the Dehn twist along $\lambda$. Then the sequence 
\[
a_{n}=\begin{cases}
T_{\lambda}^{n}\left(x\right) & n\text{ even}\\
T_{\lambda}^{n}(y) & n\text{ odd}
\end{cases}
\]
geodesically converges to $\lambda$, and no other geodesic. 

Suppose $\lambda$ is not a single simple closed curve. The above Lemma \ref{lem:grand_unicorns_geod_conv} then constructs a sequence of grand arcs $\left\{ \gamma_{i}\right\} $ that geodesically converge to a lamination $\Lambda$, which contains $\lambda$ and isolated leaves. If $\Lambda=\lambda$, then we're already done. 

Suppose $\Lambda$ contains $\lambda$ and one or two isolated leaves (which are obtained from the intersections of a grand arc $a$ that we choose, and its intersections with $\overline{N_{\epsilon}\left(\lambda\right)}$). Choose a different grand arc $a'$ disjoint from $a$, which agrees with $a$ in $\overline{N_{\epsilon}\left(\lambda\right)}$ but is not homotopic to $a$ outside (can do this unless one of the maximal ends $a$ converges to is an isolated puncture). Let $\left\{ u_{n}\right\} _{n\in\mathbb{N}}$ be the unicorn path constructed in Lemma \ref{lem:grand_unicorns_geod_conv} starting at $a$, and let $\left\{ u_{n}'\right\} _{n\in\mathbb{N}}$ be the unicorn path constructed starting at $a'$. Then the sequence 
\[
v_{n}=\begin{cases}
u_{n} & n\text{ even}\\
u_{n}' & n\text{ odd}
\end{cases}
\]
geodesically converges to $\lambda$ but no other isolated leaves.

Finally, suppose one of the maximal ends that $a$ converges to is an isolated puncture. Choose a geodesic arc $\gamma'$ (similar to $\gamma$, as in Lemma \ref{lem:grand_unicorns_geod_conv}), but starting at a different maximal end type than the isolated puncture or the end of $\gamma$ (we can do this, since the surface has at least three maximal end types). Let $\left\{ u_{n}'\right\} _{n\in\mathbb{N}}$ be the unicorn path defined by $a$ and $\gamma'$. Then defining $\left\{ v_{n}\right\} _{n\in\mathbb{N}}$ exactly as above will give us a sequence of grand arcs that geodesically converges exactly to $\lambda$.
\end{proof}

==> Modules/Old_Modules/_old__Minimisation_and_high_filling.tex <==
\section{Minimization and High Filling grand laminations}

\textcolor{red}{Abandon - minimization is basically just taking witness-filling components of derived laminations.}

Let $\lambda$ be the full limit set of a geodesically convergent sequence of grand arcs $\left\{ a_{n}\right\} _{n\in\mathbb{N}}$. 

We have the minimization process -
\[
\lambda\xrightarrow[\text{leaves}]{\text{remove isolated}}\lambda_{2}\xrightarrow[\text{leaves}]{\text{remove non-witness-filling}}\lambda_{3}.
\]

\begin{claim}
$\lambda$ high filling implies $\lambda_{3}\neq\phi$. 
\end{claim}



==> Modules/Old_Modules/_old__Surjectivity__old_.tex <==
\section{Surjectivity of $F$}

All that remains now is to show that $F$ is surjective. Once we prove this, we shall note that $F$ is a continuous bijective map from a compact space (i.e. $\mathcal{GEL}\left(\Sigma\right)$) to a Hausdorff space (i.e. $\partial\mathcal{G}\left(\Sigma\right)$), hence must be a homeomorphism. We first give an outline of the proof, and then prove the various lemmas assumed in the proof.


\begin{proof}[Outline of the proof that $F$ is surjective]
Suppose $p\in\partial\mathcal{G}\left(\Sigma\right)$. We want to construct $L\in\mathcal{GEL}\left(\Sigma\right)$ such that $F(L)=p$. Let $\left\{ c_{n}\right\} _{n\in\mathbb{N}}\subset\mathcal{G}\left(\Sigma\right)$ such that $\left[\left\{ c_{n}\right\} _{n\in\mathbb{N}}\right]=p$. Up to replacing $\left\{ c_{n}\right\} _{n\in\mathbb{N}}$ by a subsequence, we can assume that $c_{n}\to L_{0}\in\Lambda\left(\Sigma\right)$. Let $L'$ be the derived lamination of $L_{0}$ (i.e. the lamination obtained by deleting all the isolated leaves of $L'$). Then $L'$ is a union of disjoint connected components, each of which is a minimal lamination. At most one of these components $L$ fills a witness (as otherwise, the surface would have disjoint witnesses). 

We claim that at least one of the components of $L'$ fills a witness. Note that if one such component exists, it is unique (since the components fill disjoint subsurfaces, and witnesses of $\Sigma$ cannot be disjoint). Suppose for contradiction, that no component of $L'$ fills a witness (so, every component of $L'$ has a grand arc disjoint from it). We split the argument into several cases. We say that a lamination $N$ \emph{separates} \emph{two maximal end types} $e_{1}$ \emph{and} $e_{2}$ if every grand arc converging to $e_{1}$ and $e_{2}$ must intersect $N$. Similarly, we say that $N$ \emph{separates} $e_{1}$ \emph{from }$\Sigma$ if $N$ separates $e_{1}$ from every other maximal end type. 

\textbf{Case 1}: First, suppose some component $N$ of $L'$ separates at least two different maximal end types (say, $e_{1}$ and $e_{2}$) from the rest of $\Sigma$. Up to replacing $\left(x_{n}\right)_{n\in\mathbb{N}}$ with a different sequence that is Hausdorff distance at most $1$ away (by Lemma \ref{lem:dropping_perps}), we can assume that each $x_{n}$ converges to $e_{1}$ and $e_{2}$. By assumption, there is a grand arc $a$ disjoint from $N$. Let $l\in N$ be a leaf. Then for any $x_{n}$, we can find points $P_{n},Q_{n}$ of $x_{n}\cap l$ such that $x_{n}\cap a\equiv\left(P_{n}Q_{n}\right)_{x_{n}}\cap a$, and (up to choosing a slightly longer segment along $l$) such that $\left(P_{n}Q_{n}\right)_{x_{n}}$ defines a bicorn arc $y_{n}$. Then $y_{n}\in\mathcal{B}\left(x_{n},l\right)$ is disjoint from $a$. Since $x_{n}\to l$ as parametrised geodesics, we can find a $K\in\mathbb{N}$ such that $y_{n}\in\mathcal{B}\left(x_{n},x_{K}\right)$. Then 
\begin{align*}
\left(x_{n},x_{K}\right)_{a} & \leq d_{\mathrm{Haus}}\left(a,\left[x_{n},x_{K}\right]\right)+2\delta\\
 & \leq d_{\mathrm{Haus}}\left(a,\mathcal{B}\left(x_{n},x_{K}\right)\right)+2\delta+m\leq1+2\delta+m,
\end{align*}
where $m$ is the constant as in Corollary \ref{cor:unicorn_hausdorff_dist}. This contradicts that $\left[\left(x_{n}\right)_{n\in\mathbb{N}}\right]\in\partial\mathcal{G}\left(\Sigma\right)$. 

\textbf{Case 2}: Next, suppose that some component $N$ of $L'$ fills a subsurface that contains a grand arc $\alpha$. Up to replacing $\left(x_{n}\right)_{n\in\mathbb{N}}$ by a different sequence that is finite Hausdorff distance away in $\mathcal{G}\left(\Sigma\right)$, assume that $x_{0}=\alpha$ and each $x_{n}$ converges to the ends of $\alpha$. Then we can repeat the argument in the previous paragraph with $l$ a leaf of $N$ and a grand arc $a$ disjoint from $N$ to conclude that $\left(x_{n},x_{N}\right)_{a}$ is bounded. This gives us a contradiction. 

\textbf{Case 3}: Next, suppose that there is a component $N$ of $L'$ that separates a single maximal end type $e_{1}$ from the rest of $\Sigma$. Assume that $N$ does not contain a grand arc (else we're in the previous case). So, there exists a simple closed curve $\gamma$ that is disjoint from $L'$. We can then use Lemma \_\_ to replace $\left(x_{n}\right)_{n\in\mathbb{N}}$ by a new sequence, such that in the complement of $\gamma$, $L'$ is a single arc. Up to repeating this process finitely many times (and hence suitably replacing $\left(x_{n}\right)_{n\in\mathbb{N}}$ by a different sequence that converges to the same point in $\partial\mathcal{G}\left(\Sigma\right)$), we can eliminate this case.

\textbf{Case 4}: Finally, suppose $L'$ is a union of isolated leaves and minimal components that do not separate any end from $\Sigma$. In this case, by Lemma \_\_ we can construct a grand arc $\alpha$ that intersects any leaf of $L$ in at most one point. Thus, $\mathrm{diam}\left(\mathcal{B}\left(a,L\right)\right)\leq2$. This contradicts Lemma \_\_ that $\mathcal{B}\left(a,L\right)$ must be unbounded. 

Thus, in any case, $L'$ must have a component $L_{0}$ that fills a witness (i.e. $L_{0}\in\mathcal{GEL}\left(\Sigma\right)$). Finally, Lemma \ref{lem:qgeod_close_to_bicorns} says that $\left(x_{n}\right)_{n\in\mathbb{N}}$ and $F\left(L_{0}\right)$ must denote the same point in $\partial\mathcal{G}\left(\Sigma\right)$. This concludes the proof that $F$ is surjective.

\end{proof}

Now, let's build the necessary ingredients.

\begin{lem} \label{lem:dropping_perps}
Let $\left\{ x_{n}\right\} _{n\in\mathbb{N}}$ be a sequence of grand arcs, and let $e_{1}$ and $e_{2}$ be two maximal ends of different types. Then we can construct a sequence $\left\{ x_{n}'\right\} _{n\in\mathbb{N}}$ of grand arcs, such that for every $n\in\mathbb{N}$, the arc $x_{n}'$ converges to $e_{1}$ and $e_{2}$ and is disjoint from $x_{n}$.
\end{lem}

\begin{proof}
Refer to the proof of Lemma 5.6 in \cite{B-NV}. The idea is that if $x_{n}$ doesn't already converge to $e_{1}$ or $e_{2}$, then we can construct a neighbourhood of $e_{1}$ (respectively $e_{2}$) disjoint from $x_{n}$. We choose a simple arc in each of these neighbourhoods, converging to $e_{1}$ (respectively $e_{2}$) and the boundary of the corresponding neighbourhood, and extend it to intersect $x_{n}$. This gives us a new arc disjoint from $x_{n}$, which is grand by assumption.
\end{proof}

The following lemma and its proof is identical to Lemma 4.4.1 from \cite{B-W}. \textbf{ADD THE PIC FROM BW.}
\begin{lem} \label{lem:qgeod_close_to_bicorns}
Let $\kappa,\epsilon\geq0$. Let $M$ denote the $\left(\kappa,\epsilon\right)$-Morse constant of the grand arc graph. Let $\left(x_{n}\right)$ be a $\left(\kappa,\epsilon\right)$-quasi-geodesic path in the grand arc graph such that a subsequence of $\left(x_{n}\right)$ geodesically converges to some $L\in\mathcal{GEL}\left(\Sigma\right)$. Let $\left(b_{n}\right)$ denote the path in $\mathcal{B}\left(x_{0},L\right)$ as constructed in Corollary \ref{cor:coarse_conv_to_laminations}. Then $\left(x_{n}\right)$ is included in the $\left(M+2C+3\right)$-neighbourhood of $\left(b_{n}\right)$, where $C$ denotes the constant from Corollary \ref{cor:unicorn_hausdorff_dist}. 
\end{lem}

\begin{proof}
Note that $\left(b_{n}\right)$ is infinite and unbounded, by Lemma \_\_. Let $j\in\mathbb{N}$. We shall show that $x_{j}$ is in the $\left(M+2C+3\right)$-neighbourhood of $\left(b_{n}\right)$. 

Let $d_{j}$ denote the $d_{\mathcal{G}}\left(x_{0},x_{j}\right)$. Let $A\in\mathbb{N}$ such that $b_{A}$ is the first element of $\left(b_{n}\right)$ at distance $d_{j}+2M+C+1$ from $x_{0}$; that is,
\begin{itemize}
\item $d\left(x_{0},y_{A}\right)=d_{j}+2M+C+1$;
\item For every $0<k<A$, $d_{\mathcal{G}}\left(x_{0},y_{k}\right)<d_{j}+2M+C+1$.
\end{itemize}
According to Lemma \ref{lem:bicorns_for_converging_leaves}, there exists some $N$ such that the first $A$ bicorns in $\left(b_{n}\right)$ are all in $\mathcal{B}\left(x_{0},x_{N}\right)$. Consider a geodesic $\left[x_{0},x_{N}\right]$. According to Corollary \ref{cor:unicorn_hausdorff_dist}, the set $N_{1}\left(\mathcal{B}\left(x_{0},x_{N}\right)\right)$ is connected and lies in a $\left(C+1\right)$-neighbourhood of $\left[x_{0},x_{N}\right]$. Let $w\in\left[x_{0},x_{N}\right]$ be the closest point to $x_{0}$ satisfying $d\left(b_{A},w\right)\leq C+1$. For every $n\leq A$, $y_{n}$ is $\left(C+1\right)$-close to $\left[x_{0},w\right]$. Hence, $\left[x_{0},w\right]$ is in the $\left(2C+3\right)$-neighbourhood of $\left(b_{n}\right)$. 

On the other hand, $x_{j}$ is in the $M$-neighbourhood of $\left[x_{0},x_{N}\right]$. Let $z\in\left[x_{0},x_{N}\right]$ such that $d\left(x_{j},z\right)\leq M$. The triangle inequality gives us that $d\left(x_{0},z\right)\leq d_{j}+M$. At the same time, the triangle inequality gives us $d\left(x_{0},y_{A}\right)\leq d\left(x_{0},w\right)+d\left(y_{A},w\right)$, so that $d\left(x_{0},w\right)\geq d_{j}+2M$. Thus, $z\in\left[x_{0},w\right]$. Thus, $x_{j}$ is distance at most $M$ from $z$, and $z$ distance at most $\left(2C+3\right)$ from some point in $\left(b_{n}\right)$. This concludes the proof.
\end{proof}

\begin{lem}
Suppose $L$ is a lamination on $\Sigma$, and let $L'$ be the derived lamination. Suppose that there exists a grand arc $\alpha$ disjoint from $L'$. Then we can construct a grand arc $\beta$ which intersects every leaf of $L$ at most once.
\end{lem}

\begin{lem}
Suppose that $\left\{ x_{n}\right\} _{n\in\mathbb{N}}$ is a sequence of grand arcs that converges to a grand ending lamination $L$. Then 
\[
\mathcal{B}\left(x_{0},L\right)=\cup_{N\in\mathbb{N}}\cap_{n\geq N}\mathcal{B}\left(x_{0},x_{n}\right).
\]
\end{lem}


==> Modules/Old_Modules/_old__Unicorns.Bicorns.tex <==
\section{Unicorn Paths in $\mathcal{GL}(\Sigma)$}
Define unicorns as in \cite{B-NV}.

From \cite{B-NV}, we get :
\begin{lem}
Let $\Sigma$ be a surface with $\mathcal{S}\left(\Sigma\right)\geq3$. Let $\alpha,\beta\in\mathcal{G}\left(\Sigma\right)$. Then:
\begin{enumerate}
\item The subgraph of $\mathcal{G}\left(\Sigma\right)$ spanned by $N_{1}\left(\mathcal{U}_{G}\left(\alpha,\beta\right)\right)$ is connected.
\item If $d_{\mathcal{G}}\left(\alpha,\beta\right)\leq1$, then $\mathrm{diam}\left(N_{1}\left(\mathcal{U}_{G}\left(\alpha,\beta\right)\right)\right)\leq3$.
\end{enumerate}
\end{lem}

\begin{defn}
The \emph{grand unicorns} between a grand arc $a$ and a sequence $\left\{ x_{n}\right\} _{n\in\mathbb{N}}\subset \mc G(\Sigma)$ is the collection 
\[
\mathcal{U}_{G}\left(a,\left\{ x_{n}\right\} _{n\in\mathbb{N}}\right):=\bigcup_{n\in\mathbb{N}}\mathcal{U}_{G}\left(a,x_{n}\right).
\]
\end{defn}

\begin{lem}
Let $a\in\mathcal{G}\left(\Sigma\right)$ and $\Lambda\in\mathcal{GL}\left(\Sigma\right)$. Suppose $\left\{ x_{n}\right\} _{n\in\mathbb{N}},\left\{ y_{n}\right\} _{n\in\mathbb{N}}\subset\mathcal{G}\left(\Sigma\right)$ such that $x_{n}\to\Lambda$ and $y_{n}\to\Lambda$. Then there exists $C>0$ such that 
\[
d_{\mathrm{Haus}}\left(\mathcal{U}_{G}\left(a,\left\{ x_{n}\right\} _{n\in\mathbb{N}}\right),\mathcal{U}_{G}\left(a,\left\{ y_{n}\right\} _{n\in\mathbb{N}}\right)\right)<C.
\]
\end{lem}

\textcolor{red}{Pause - Carolyn's idea: instead of working with unicorns, what if we just work with geodesically converging sequences of grand arcs? Given a grand lamination, we already have an associated sequence of grand arcs for the lamination...}

==> Modules/Old_Modules/_old__k-agrees-with.tex <==
\section{Equators and $k$-agrees-with convergence.}

\textcolor{red}{In this section, we want to define equators and $k$-agrees-with convergence, and show that this is equivalent to geodesic convergence.}

\textcolor{red}{All of this section is copied from version 4, and needs to be edited.}

As in Theorem 3.0.1 in \cite{B-W_2}, we can construct a fundamental domain for the $\pi_{1}\left(\Sigma\right)$-action on the universal cover $\mathbb{H}^{2}$ of $\Sigma$, whose vertices are all in $\partial\mathbb{H}^{2}$. 

\textcolor{blue}{Fill in details here}


\begin{defn}
Let $\lambda,\mu$ be two simple geodesics on $\Sigma$. We say that $\mu$
\emph{$k$-agrees-with} $\lambda$ for some $k\in\mathbb{N}$ if we can choose
lifts $\tilde{\lambda}$ of $\lambda$ and $\tilde{\mu}$ of $\mu$, each
intersecting $P_{0}$, so that they intersect the same first $k$ equators on
either side of $\tilde{\lambda}(0)$ and $\tilde{\mu}(0)$. 
\end{defn}

\begin{lem}
Let $\left\{ \lambda_{i}\right\} _{i\in\mathbb{N}}$ be a sequence of simple geodesics on $\Sigma$.  The following are equivalent:
\begin{enumerate}
\item The sequence $\left\{ \lambda_{i}\right\} _{i\in\mathbb{N}}$ geodesically converges to some grand lamination $\Lambda$.
\item For every $k\in\mathbb{N}$, there exists $N\in\mathbb{N}$ such that $\lambda_{i}$ $k$-agrees-with $\lambda$ for all $i\geq N$, for any $\lambda \in \Lambda$. 
\end{enumerate}
\end{lem}

\begin{proof}
A sequence of lifts $\tilde{\lambda}_{i}$ cover-converges to a geodesic $\tilde{\lambda}$ if and only if they intersect the same set of fundamental domains for longer and longer along $\tilde{\lambda}_{i}$ as $i$ increases, which is the same as saying that $\lambda_{i}$ $k$-agrees-with $\lambda$ for larger and larger $k$. This shows that (2) and (3) are equivalent.

\textcolor{blue}{Needs more justification.}
\end{proof}

\textbf{Remark} - When doing $k$-agrees-with convergence, we want to specify a parametrization for the limiting geodesic (just as we do for geodesic convergence).

==> Modules/Old_Modules/_old__k-filling_business.tex <==
\section{$k$-filling and high filling grand laminations.}
\begin{defn}
Let $\Lambda$ be a grand lamination. 
\begin{enumerate}
    \item We say that $\Lambda$ is \textit{arc-filling} if it intersects every grand arc transversely.
    \item We say that $\Lambda$ is \textit{$1$-filling} if there exists a grand arc disjoint from every leaf of $\Lambda$.
    \item We say that $\Lambda$ is \textit{$k$-filling} for $k\geq 2$ if it is not $l$ filling for any $l < k$ and is disjoint 
    from a grand lamination that is $(k-1)$-filling.
    \item We say that $\Lambda$ is \textit{high-filling} if it is not $k$-filling 
    for any $k\in\mathbb{N}$.
    \item We say that $\Lambda$ is \textit{witness-filling} if for every witness $W$, (some leaf of) $\Lambda$ intersects $W$ transversely.
    \end{enumerate}
\end{defn}

\begin{lem}
    An arc-filling grand line is witness-filling.
\end{lem}

\begin{proof}
Suppose an arc-filling grand lamination $\Lambda$ is disjoint from a witness $W$. Then $\Lambda$ is contained in one of the components of $\Sigma \backslash W$, each of which is a surface with exactly one maximal end type. Since $\Sigma$ has at least three maximal end types, there are at least two components $C_{1}$ and $C_{2}$ of $\Sigma\backslash W$ which are disjoint from $\Lambda$. Then $W\cup C_{1}\cup C_{2}$ is a surface containing two of the maximal end types of $\Sigma$, and every grand arc in $W\cup C_{1}\cup C_{2}$ between these two maximal end types must be disjoint from $\Lambda$.
\end{proof}

\begin{lem}\label{lem:high_filling_unbdd}
Suppose $\Lambda$ is a high-filling grand lamination, let $a$ be a grand arc, and suppose $\left\{ x_{n}\right\} _{n\in\mathbb{N}}\subset\Gamma_{\mathrm{grand}}\left(\Sigma\right)$ converges to $\Lambda$. Then $\lim_{n\to\infty}d\left(a,x_{n}\right)=\infty$.
\end{lem}

\begin{proof}
Suppose for contradiction, that there exists some $R\in\mathbb{N}$ and an infinite subsequence $\left\{ x_{n}'\right\} _{n\in\mathbb{N}}\subset\left\{ x_{n}\right\} _{n\in\mathbb{N}}$ such that $d_{\mathcal{G}}\left(a,x_{n}'\right)\leq R$ for all $n\in\mathbb{N}$. For every $n$, let $y_{i}^{n}\in\mathcal{G}\left(\Sigma\right)$ for $1\leq i\leq R$ define a path between $a$ and $x_{n}'$, so that each $y_{i}^{n}$ is disjoint from $y_{i\pm1}^{n}$, $y_{0}^{n}=a$ and $y_{R}^{n}=x_{n}'$. By Proposition \ref{prop:grand_laminations_compact}, a subsequence of each sequence $\left(y_{i}^{n}\right)_{n\in\mathbb{N}}$ converges to a grand lamination $\Lambda_{i}$ (where $\Lambda_{0}=\left\{ a\right\} $ and $\Lambda_{R}=\Lambda$). Moreover, by Lemma \ref{lem:disjt_convergence}, each $\Lambda_{i}$ is disjoint from $\Lambda_{i\pm1}$. This shows that $\Lambda$ is at most $R$-filling, which is a contradiction.
\end{proof}

\begin{lem} \label{lem:k-agrees-with_distance}
Let $a,x\in\mathcal{G}\left(\Sigma\right)$. Fix a parametrisation on $x$.Then there exists a $k\in\mathbb{N}$ and such that for any $y\in\mathcal{G}\left(\Sigma\right)$ which $k$-agrees-with $x$, we have 
\[
d_{\mathcal{G}}\left(a,y\right)\geq d_{\mathcal{G}}\left(a,x\right)-3.
\]
\end{lem}

\begin{proof}
Pick a witness $W$ large enough such that $x\cap W$ is a single arc. Pick $k$ large enough so that if $y$ $k$-agrees-with $x$, then $x\cap W\subset y\cap W$. Then $d_{\mathcal{G}}\left(x,y\right)\leq3$, and the conclusion follows.
\end{proof}
\begin{prop}
Suppose $\Lambda$ is a high-filling grand lamination, and $\left\{ x_{n}\right\} _{n\in\mathbb{N}}$ and $\left\{ y_{m}\right\} _{m\in\mathbb{N}}$ are two sequences of grand arcs that both geodesically converge to $\Lambda$. Let $a\in\mathcal{G}\left(\Sigma\right)$ be a fixed base point. Then we have 
\[
\lim_{m,n\to\infty}\left(x_{n},y_{m}\right)_{a}=\infty,
\]
where $\left(x_{n},y_{m}\right)_{a}$ is the Gromov product in $\mathcal{G}\left(\Sigma\right)$. 
\end{prop}

\begin{proof}
Recall that 
\[
\left(x_{n},y_{m}\right)_{a}\geq d_{\mathcal{G}}\left(a,\left[x_{n},y_{m}\right]\right)-2\delta,
\]
where $\left[x_{n},y_{m}\right]$ is a geodesic in $\mathcal{G}\left(\Sigma\right)$ joining $x_{n}$ and $y_{m}$. Since $N_{1}\left(\mathcal{B}\left(x_{n},y_{m}\right)\right)$ is a uniform quasi-geodesic \textcolor{blue}{(Needs justification)}, we get 
\[
\left(x_{n},y_{m}\right)_{a}\geq d_{\mathcal{G}}\left(a,N_{1}\left(\mathcal{B}_{\mathrm{path}}\left(x_{n},y_{m}\right)\right)\right)-2\delta-C
\]
for some constant $C>0$. We want to show that as $m,n\to\infty$, points in $\mathcal{B}_{\mathrm{path}}\left(x_{n},y_{m}\right)$ are all going further from $a$.

Since $\left\{ x_{n}\right\} _{n\in\mathbb{N}}$ and $\left\{ y_{m}\right\}
_{m\in\mathbb{N}}$ are unbounded (by Lemma \ref{lem:high_filling_unbdd}), for
any $R>0$, we can choose $N,M\in\mathbb{N}$ such that for all $n\geq N$ and
$m\geq M$, we have $d_{\mathcal{G}}\left(a,x_{n}\right)\geq R$ and
$d_{\mathcal{G}}\left(a,y_{m}\right)\geq R$ respectively. Moreover, for any
$k\in\mathbb{N}$, we can choose possibly larger $N,M$ such that $x_{n}$ and
$y_{m}$ both $k$-agree-with $\lambda$ (and hence each other), for $n\geq N$ and
$m\geq M$. Furthermore, we can construct a path in
$\mathcal{G}\left(\Sigma\right)$ in the 1-neighbourhood of bicorn arcs between
$x_{n}$ and $y_{m}$, \abn{It's not clear that taking a bicorn of $x_n$ and $y_n$ indeed gives something that $k$-agrees with $\Lambda$.} and every bicorn $b$ in this path would $k$-agree-with
$x_{n}$ and $y_{m}$.

Finally, by Lemma \ref{lem:k-agrees-with_distance}, there is a $k$ large enough so that if any grand arc $g$ $k$-agrees-with $x_{n}$, then 
\[
d_{\mathcal{G}}\left(a,g\right)\geq d_{\mathcal{G}}\left(a,x_{n}\right)-3\geq R-3.
\]
Thus, as $m,n\to\infty$, so does $\left(x_{n},y_{m}\right)_{a}$. 
\end{proof}

\begin{lem} (Bavard-Walker 4.4.1)
Suppose that $x_n$ is a (quasi-geodesic \abn{necessary?}) sequence that geodesically converges to a high-filling grand lamination $\Lambda$ then for any basepoint $a \in \mathcal{G}(\Sigma)$, there exists some $R > 0$ such that $\mathcal{N}_R(\mathcal{B}(a, \Lambda)) \supset \{x_n\}$
\end{lem}
\abn{This is similar to Lemma 3.7. We need to prove that if $x_n, y_n \to \Lambda$, then $\cup_n \mathcal{B}(a, x_n)$ and $\cup_n \mathcal{B}(a, y_n)$ are uniform distance apart. Then, we'd want to show that $\mathcal{B}(a, y_n)$ is uniformly close to a quasi-geodesic}

(cf. BW 3.4.7)

\abn{One idea we had was to look at convergence to the boundary of prescribed arc graphs of finite-type exhaustions of the surface}

==> Modules/linear-connectivity.tex <==
\subsection{Connected spheres in $\mathcal{G}(\Sigma)$}

In order to prove that $\partial\mathcal{G}\left(\Sigma\right)$ is linearly connected, we shall use the machinery developed by Wright (see Proposition 2.2 in \cite{Wright}) and improved by Long and Tan in \cite{LT}. In what follows, for $a\in\mathcal{G}(\Sigma)$, and $r\in\mathbb{N}$, we define $$S_{a}(r)=\left\{ x\in\mathcal{G}\left(\Sigma\right)\mid d_{\mathcal{G}}\left(a,x\right)=r\right\} $$ and $$B_{a}(r)=\left\{ y\in\mathcal{G}\left(\Sigma\right)\mid d_{\mathcal{G}}\left(a,y\right)\leq r\right\}.$$ 
\begin{prop}[Proposition 2.11 in \cite{LT}] \label{prop:boundary_lin_con}
Let $\Gamma$ be a Gromov hyperbolic simplicial graph and let $o\in\Gamma$ be a base point. Suppose that the following conditions are satisfied:

\begin{enumerate}
\item Every vertex of $\Gamma$ is adjacent to a point of $\Gamma$ that is at least $1$ farther from $o$.
\end{enumerate}

Moreover, suppose there is some $D>0$ such that for all $r\geq0$:

\begin{enumerate}\addtocounter{enumi}{1}
\item For every $z\in S_{o}(r)$ and $x,y\in S_{o}\left(r+1\right)\cap B_{z}(1)$, there exists a path 
\[
x=x_{0},x_{1},\dots,x_{l}=y
\]
with 
\[
x_{i}\in\left(\Gamma-B_{o}\left(r\right)\right)\cap B_{x}\left(D\right)
\]
for $0\leq i\leq l$.
\item For every adjacent pair $x,y\in S_{o}(r)$ there exists a path 
\[
x=x_{0},x_{1},\dots,x_{k}=y
\]
with
\[
x_{i}\in\left(\Gamma-B_{o}\left(r\right)\right)\cap B_{x}(D)
\]
for $0<i<l$.
\end{enumerate}
\end{prop}

We shall apply Proposition \ref{prop:boundary_lin_con} to the grand arc graph, for an infinite-type surface with at least $4$ elements in the grand splitting. Corollary \ref{cor:no_dead_ends} already proves the first assumption of the theorem. The following two lemmas will prove the second and third condition, respectively.

\begin{lem}
\label{lem:path_outside_sphere}Suppose $\Sigma$ is an infinite-type surface with at least $4$ elements in the grand splitting, and let $o\in\mathcal{G}\left(\Sigma\right)$ be a fixed base point. Suppose $z\in S_{o}(r)$. Then the set $S_{o}\left(r+1\right)\cap B_{z}(1)$ is connected.
\end{lem}

\begin{lem}\label{lem:sphere_connected}
    For any two grand arcs $p,q\in S_{o}(r)$ that are adjacent, there exists a grand arc $s\in S_{o}(r+1)$ disjoint from both $p$ and $q$.
\end{lem}

The proof of Lemma \ref{lem:path_outside_sphere} follows the proof of Lemma 7.2 from \cite{Wright}, with the added advantage that we don't need to worry about surfaces with ``low or medium complexity''. We start with a compact witness $W\subset\Sigma$ large enough so that $o\cap W$ and $z\cap W$ are connected (so that $Y=W\backslash z$ is a partial witness) and that $W$ has sufficiently high complexity. We may further assume that $o$ and $z$ are disjoint outside $W$. Define 
\[
\mathcal{O}_{W}(z)=\left\{ x\in S_{o}\left(r+1\right)\cap B_{z}(1)\mid x\cap W\text{ is connected and }d_{Y}\left(o,x\right)> M+K\right\} ,
\]
where $M$ is the constant from Theorem \ref{thm:BGI}, and $K$ is the quasi-geodesic constant of bicorn paths. We shall first construct a path in $S_{o}\left(r+1\right)\cap B_{z}(1)$ between any two points in $\mathcal{O}_{W}(z)$, and then construct a path from any other point in $S_{o}\left(r+1\right)\cap B_{1}\left(z\right)$ to some point in $\mathcal{O}_{W}(z)$.

\textcolor{red}{Pause - need to be careful in the lemmas below. We're cutting two grand arcs, and the resulting subsurface need not be a partial witness. This is resolved if surface has at least 5 max ends, or maybe something smart works for 4. Also need to develop a version of BGI for prescribed arc graphs / arc graphs of subsurfaces.}

\textcolor{blue}{Update - nothing to do with 5 max ends - need that the two arcs you're cutting don't start and end at same boundaries...}

\begin{lem}
\label{lem:getting_to_O(K)}Let $x\in S_{o}\left(r+1\right)\cap B_{z}(1)$. Then there exists a path $x=x_{0},x_{1},\dots,x_{k}=y$ in $S_{o}\left(r+1\right)\cap B_{z}(1)$ for some $y\in\mathcal{O}_{W}(z)$ (for $W$ as defined in the previous paragraph).
\end{lem}

\begin{proof}
Let $b_{1},b_{2}$ denote the components of $\partial W$ which $x$ intersects. Up to choosing a different grand arc in $S_{o}\left(r+1\right)\cap B_{z}(1)$ which is disjoint from $x$, we may assume that $z$ also intersects $\partial W$ in $b_{1},b_{2}$. We may also assume that $x$ is disjoint from $o$ outside $W$ \textbf{(need to elaborate on all the choices)}. Then note that $W\backslash\left(x\cup z\right)$ has at least one connected component which is a partial witness (there are at least three elements of the grand splitting that are not separated from each other by $x\cup z$) - call this component $V$. Let $x_{1}\in\mathcal{G}\left(\Sigma\right)$ such that $x_{1}\cap W$ is a single arc from $b_{1}$ to $b_{2}$, $x_{1}\equiv x$ outside $W$, and $d_{V}\left(o,x_{1}\right)>M$. Then by Theorem \ref{thm:BGI}, every geodesic in $\mathcal{G}\left(\Sigma\right)$ joining $o$ and $x_{1}$ has a grand arc which is disjoint from $V$ (hence, disjoint from $x\cup z$). Thus, $x_{1}\in S_{o}\left(r+1\right)\cap S_{z}(1)$. 

Inductively, suppose $x_{i}\in S_{o}\left(r+1\right)\cap B_{z}(1)$ is constructed, where $x_{i}$ also connects $b_{1}$ and $b_{2}$ in $W$ and $x_{i}\equiv x$ outside $W$. Using the argument above, we can construct $x_{i+1}\in S_{o}\left(r+1\right)\cap S_{z}(1)$ with $d_{V_{i}}\left(o,x_{i+1}\right)>M$, where $V_{i}$ is a component of $W\backslash\left(x_{i}\cup z\right)$ which is a partial witness. Then $x_{i+1}\in S_{o}\left(r+1\right)\cap S_{1}(z)$, and is disjoint from $x_{i}$. On the other hand, $\Sigma_{i}=\Sigma\backslash x_{i}$ is also an infinite-type surface with at least $4$ maximal ends, so that $V$ is a partial witness in $\Sigma_{i}$. Then by Theorem \ref{thm:BGI} in $\Sigma_{i}$, $d_{V}\left(o,x_{i+1}\right)>M$ implies that any geodesic in $\mathcal{G}\left(\Sigma_{i}\right)$ joining $o$ and $x_{i+1}$ must go through $x_{i}$, implying that $d_{Y}(o,x_{i+1})=d_{Y}\left(o,x_{i}\right)+1$. Repeating this process at most $M+K$ times, we obtain $x_{M+K}\in\mathcal{O}_{W}(z)$. \textbf{(Here we should argue using BGI in $Y$ instead of $\Sigma_{i}$, so need to appropriately edit BGI).}
\end{proof}
%

\textcolor{red}{No, needs more work. $x,y$ large distance in $Y$ does not mean each bicorn between them is large distance.}

\begin{proof}[Proof of Lemma \ref{lem:path_outside_sphere}]
Let $x,y\in S_{o}\left(r+1\right)\cap B_{z}(1)$. First, assume that $x,y\in\mathcal{O}_{W}(z)$ (up to choosing $W$ large enough). Since $x,y$ project to connected arcs in $W$, every grand arc in $\mathcal{B}\left(x,y\right)$ projects to a connected arc in $W$ disjoint from $z$. Since $N_{1}\left(\mathcal{B}\left(x,y\right)\right)$ is connected (by Lemma \ref{lem:finite_bicorns_connected}), we get a bicorn path $x=x_{0},x_{1},\dots,x_{k}=y$. \sout{Moreover, by our assumption, $d_{Y}\left(x_{i},o\right)>M$ for each $i$, so that $x_{i}\in S_{o}\left(r+1\right)$ as desired.} Finally, Lemma \ref{lem:getting_to_O(K)} states that any points outside $\mathcal{O}_{W}(z)$ can be connected to some point in $\mathcal{O}_{W}(z)$ via a path in $S_{o}\left(r+1\right)\cap B_{z}(1)$. Concatenating these paths with the path in $\mathcal{O}_{W}(z)$, we can obtain a path in $S_{o}(r+1)\cap B_{z}(1)$ between any two points $x,y$. 
\end{proof}


==> Old_versions/Rough.tex <==
To this extent, first note that for any $\epsilon>0$ and a grand line $\lambda$, every connected component of $\Sigma-N_{\epsilon}\left(\lambda\right)$ is a surface (even though connected components of $\Sigma-\lambda$ need not be surfaces). If we further assume that $\lambda$ is arc-filling (i.e. $\lambda$ intersects every grand arc transversely), then any connected component of $\Sigma-N_{\epsilon}\left(\lambda\right)$ may have at most one maximal end type. This leads us to the following definition - 
\begin{defn}
Let $\lambda$ be an arc-filling grand line. We say that a maximal end class is \emph{cut off by $\lambda$} if an open neighbourhood of this maximal end class is contained in a component of $\Sigma-N_{\epsilon}\left(\lambda\right)$ (for any $\epsilon>0$). Else, we must have that $\lambda$ has limit points to this maximal end class. We denote by $E_{c}\left(\lambda\right)$ the maximal ends cut off by $\lambda$, and $E_{l}\left(\lambda\right)$ the maximal end types that $\lambda$ limits to. 
\end{defn}

Note that the above definition is independent of the choice of $\epsilon>0$. This gives us a splitting 
\[
\mathcal{M}\left(\Sigma\right)=E_{c}\left(\lambda\right)\sqcup E_{l}\left(\lambda\right).
\]
We shall have several cases based on the number of maximal ends of each type. Note that by definition of grand lines, $\#E_{l}\left(\lambda\right)\geq1$. 
\begin{lem} \label{lem:intersection_at_end}
Suppose an arc-filling grand line $\lambda$ has limit points to a maximal end type $e$. Then there exists a grand arc $a$ such that $\left\{ a\cap\lambda\right\} $ has limit points to $e$. 
\end{lem}

\begin{proof}
Consider an open neighbourhood $U$ of $e$, which is an infinite-type surface with one maximal end type. We can further assume that $U$ shares one boundary simple closed curve with $\Sigma$. Consider a compact exhaustion of $U$, given by $K_{1}\subset K_{2}\subset\dots$ s.t. $\cup_{i\in\mathbb{N}}K_{i}=U$. Since $\lambda$ has limit points to $e$, for each $i>0$, $\lambda\cap\left(K_{i}\backslash K_{i-1}\right)$ is non-empty. In particular, $\lambda\cap\left(K_{i}\backslash K_{i-1}\right)$ must contain at least one ``vertical arc'', connecting a component of $\partial K_{i-1}$ to a different component of $\partial K_{i}$. \textbf{TO BE COMPLETED}.
\end{proof}
%

\begin{cor}
Suppose $\lambda$ is an arc-filling grand lines, with $E_{l}\left(\lambda\right)\geq2$. Then we can choose $x\in\mathcal{G}\left(\Sigma\right)$ such that for any arc-filling grand line $\lambda'$ disjoint from $\lambda$, we have 
\[
\mathcal{B}\left(x,\lambda'\right)\subset N_{1}\left(\mathcal{B}\left(x,\lambda\right)\right).
\]
\end{cor}

\begin{proof}
Let $e_{1},e_{2}$ be two of the maximal end types that $\lambda$ has limit points to. By using Lemma \ref{lem:intersection_at_end} twice, we can construct a grand arc $x$ such that $x\cap\lambda$ limits to both $e_{1}$ and $e_{2}$. Thus, for any two points $P,Q$ on $x$, we can find points $P',Q'\in x\cap\lambda$ such that $P'-P-Q-Q'$ along $x$. As a result, for any grand line $\lambda'$, for any bicorn in $\mathcal{B}\left(x,\lambda'\right)$, Lemma \ref{lem:bicorns_dist_1} is satisfied and we can find a bicorn in $\mathcal{B}\left(x,\lambda\right)$ which is distance $\leq1$ away.
\end{proof}
%

\begin{prop}
Suppose $\lambda,\lambda'$ are disjoint arc-filling grand lines, with $E_{c}\left(\lambda\right)\cap E_{c}\left(\lambda'\right)\geq3$. Then we can find $x\in\mathcal{G}\left(\Sigma\right)$ such that one of $\mathcal{B}\left(x,\lambda\right)$ and $\mathcal{B}\left(x,\lambda'\right)$ is contained in a $1$-neighbourhood of the other.
\end{prop}

\begin{proof}
Let $e_{1},e_{2},e_{3}\in E_{c}\left(\lambda\right)\cap E_{c}\left(\lambda'\right)$. Let $\alpha_{1},\alpha_{2},\alpha_{3}\in\partial N_{\epsilon}\left(\lambda\right)$ be separating simple closed curves that cut off an open neighbourhood of $e_{1},e_{2},e_{3}$ respectively. Similarly, let $\beta_{1},\beta_{2},\beta_{3}\in\partial N_{\epsilon}\left(\lambda\right)$ be separating simple closed curves that cut off open neighbourhoods of $e_{1},e_{2},e_{3}$ respectively. We make cases depending on the position of these curves in $\Sigma$. 
\begin{casenv}
\item Suppose for some $i,j\in\left\{ 1,2,3\right\} $, we have $\alpha_{i}\cap\beta_{i}\neq\phi$ and $\alpha_{j}\cap\beta_{j}\neq\phi$. 

In this case, we can choose $x\in\mathcal{G}\left(\Sigma\right)$ converging to $e_{i}$ and $e_{j}$, such that $x$ intersects each of $\alpha_{i},\alpha_{j},\beta_{i},\beta_{j}$ exactly once, and $x\cap\beta_{i},x\cap\beta_{j}$ are between $x\cap\alpha_{i},x\cap\alpha_{j}$ along $x$. This gives us that every point of $x\cap\lambda'$ (along $x$) is contained between points of $x\cap\lambda$. As a result, we get that $\mathcal{B}\left(x,\lambda'\right)\subset N_{1}\left(\mathcal{B}\left(x,\lambda\right)\right)$. 
\item Suppose for some $i,j\in\left\{ 1,2,3\right\} $, we have $\alpha_{i}\cap\beta_{i}\neq\phi$, and $\alpha_{j}\cap\beta_{j}=\phi$. 

In this case, we must have that either $\alpha_{j}\subset\Sigma-N_{\epsilon}\left(\lambda'\right)$, or $\beta_{j}\subset\Sigma-N_{\epsilon}\left(\lambda\right)$. Without loss of generality, assume the former (else, switch the roles of $\lambda$ and $\lambda'$ in the following argument). Choose $x\in\mathcal{G}\left(\Sigma\right)$ converging to $e_{i}$ and $e_{j}$, such that $x$ intersects each of $\alpha_{i},\alpha_{j},\beta_{i},\beta_{j}$ exactly once, and when oriented from $e_{i}$ to $e_{j}$, $x\cap\alpha_{i}$ is before $x\cap\beta_{i}$ along $x$. Then once again, every point of $x\cap\lambda'$ (along $x$) is contained between points of $x\cap\lambda$. As a result, we get that $\mathcal{B}\left(x,\lambda'\right)\subset N_{1}\left(\mathcal{B}\left(x,\lambda\right)\right)$. 
\item Else, we have $\alpha_{1}\cap\beta_{1}=\phi$, $\alpha_{2}\cap\beta_{2}=\phi$ and $\alpha_{3}\cap\beta_{3}=\phi$. 

Note that for any $i\in\left\{ 1,2,3\right\} $, either $\alpha_{i}\subset\Sigma-N_{\epsilon}\left(\lambda'\right)$ or $\beta_{i}\subset\Sigma-N_{\epsilon}\left(\lambda\right)$. Thus, we can always find $i,j\in\left\{ 1,2,3\right\} $ such that either $\Sigma-N_{\epsilon}\left(\lambda'\right)$ contains both $\alpha_{i}$ and $\alpha_{j}$ or $\Sigma-N_{\epsilon}\left(\lambda\right)$ contains both $\beta_{i}$ and $\beta_{j}$. In the first case, we can once again construct a grand arc $x$ converging to $e_{i}$ and $e_{j}$ such that every point of $x\cap\lambda'$ (along $x$) is contained between points of $x\cap\lambda$. As a result, we get that $\mathcal{B}\left(x,\lambda'\right)\subset N_{1}\left(\mathcal{B}\left(x,\lambda\right)\right)$. Similarly, if $\Sigma-N_{\epsilon}\left(\lambda\right)$ contains both $\beta_{i}$ and $\beta_{j}$, then we get $\mathcal{B}\left(x,\lambda\right)\subset N_{1}\left(\mathcal{B}\left(x,\lambda'\right)\right)$. 

\end{casenv}
Thus, in any case, we can find $x\in\mathcal{G}\left(\Sigma\right)$ such that one of $\mathcal{B}\left(x,\lambda\right)$ and $\mathcal{B}\left(x,\lambda'\right)$ is contained in the $1$-neighbourhood of the other.
\end{proof}


We have thus shown that if $\lambda,\lambda'$ are disjoint arc-filling grand lines, then $\mathcal{B}\left(a,\lambda\right)$ and $\mathcal{B}\left(a,\lambda'\right)$ define the same point in $\partial\mathcal{G}\left(\Sigma\right)$ if $E_{l}\left(\lambda\right)\geq2$, $E_{l}\left(\lambda'\right)\geq2$ or if $E_{c}\left(\lambda\right)\cap E_{c}\left(\lambda'\right)\geq3$. Moreover, by the definition of grand lines, we have $E_{l}\left(\lambda\right),E_{l}\left(\lambda'\right)\geq1$. This leaves us with only three other cases to consider, which we shall cover below.

\begin{lem}
Suppose $\Sigma$ has four maximal end types $e_{1},e_{2},e_{3},e_{4}$. Suppose $\lambda,\lambda'$ are disjoint arc-filling grand lines in $\Sigma$. Suppose $e_{1},e_{2}\in E_{c}\left(\lambda\right)\cap E_{c}\left(\lambda'\right)$, $e_{3}\in E_{c}\left(\lambda\right)\cap E_{l}\left(\lambda'\right)$ and $e_{4}\in E_{l}\left(\lambda\right)\cap E_{c}\left(\lambda'\right)$. Then there exists $x\in\mathcal{G}\left(\Sigma\right)$ such that one of $\mathcal{B}\left(x,\lambda\right)$ and $\mathcal{B}\left(x,\lambda'\right)$ is contained in the $1$-neighbourhood of the other.
\end{lem}

\begin{proof}
Let $\alpha_{1},\alpha_{2}\in\partial N_{\epsilon}\left(\lambda\right)$ and $\beta_{1},\beta_{2}\in\partial N_{\epsilon}\left(\lambda'\right)$ be separating simple closed curves cutting off open neighbourhoods of $e_{1},e_{2}$ respectively. Using the cases covered in the proof of Proposition \_\_, if $\alpha_{1}\cap\beta_{1}\neq\phi$, $\alpha_{2}\cap\beta_{2}\neq\phi$, then the result is true. 

Suppose $\alpha_{1}\subset\Sigma-N_{\epsilon}\left(\lambda'\right)$. Then we can construct a grand arc $x$ converging to $e_{1}$ and $e_{4}$, such that points of $x\cap\lambda$ limit to $e_{4}$. Thus, by Lemma \_\_, we get $\mathcal{B}\left(x,\lambda'\right)\subset N_{1}\left(\mathcal{B}\left(x,\lambda\right)\right)$. Else, we have $\beta_{1}\subset\Sigma-N_{\epsilon}\left(\lambda\right)$. Then we can construct a grand arc $x$ converging to $e_{1}$ and $e_{3}$, such that points of $x\cap\lambda'$ limit to $e_{3}$. Thus, by Lemma \_\_, we get $\mathcal{B}\left(x,\lambda\right)\subset N_{1}\left(\mathcal{B}\left(x,\lambda'\right)\right)$.
\end{proof}

\begin{lem}
The map $\psi ^{-1}$ is continuous.
\end{lem}

\begin{proof}
Note that even though $\mathcal{G}\left(\Sigma\right)$ is not proper, $\\mathcal{G}\left(\Sigma\right)$ is first-countable (see \_\_). So to show that $\psi ^{-1}$ is continuous, it suffices to show that if $\left\{ P_{i}\right\} _{i\in\mathbb{N}}$ is a sequence of points in $\partial\mathcal{G}\left(\Sigma\right)$ that converges in the visual topology to $P_{0}$, then for all $i$, we can find $\mu_{i}\in\Phi^{-1}\left(P_{i}\right)$ such that $\mu_{i}\xrightarrow{\mathrm{CHCCS}}\mu_{0}$. Let $\mu_{i}\in\Phi^{-1}\left(P_{i}\right)$. By Lemma \ref{lem:CHCCS_seq_cpct}, up to choosing a subsequence, we can find $\mu_{0}\in\mathcal{H}\left(\Sigma\right)$ such that $\mu_{i}\xrightarrow{\mathrm{CHCCS}}\mu_{0}$. We shall show that $\Phi\left(\mu_{0}\right)=P_{0}$. 

Using Lemma \ref{lem:bicorn_paths}, we can choose $\left\{ a_{i,n}\right\} _{i\in\mathbb{N}}\subset\mathcal{B}\left(a,\mu_{i}\right)$ such that $a_{i,n}\xrightarrow{\mathrm{CHCCS}}\mu_{i}'$ for some $\mu_{i}'\in\Phi^{-1}\left(\mu_{i}\right)$. Then $\left\{ a_{i,n}\right\} _{i\in\mathbb{N}}$ defines an unparametrised quasi-geodesic that limits to $P_{i}=\Phi\left(\mu_{i}\right)$. By the hyperbolicity of $\mathcal{G}\left(\Sigma\right)$, and Corollary \ref{cor:unicorn_hausdorff_dist} (that bicorn paths are unparametrised uniform quasi-geodesics), there exists a constant $C=C\left(\delta\right)$ such that $\forall r>0$, $\exists n_{r}\in\mathbb{N}$ such that $a_{j,n_{r}}\in N_{C}\left(\left\{ a_{i,0}\right\} _{i}\right)$ for any $j$ with $d\left(a,a_{j,n_{r}}\right)\leq r$. Note that choosing a larger $n_r$ also makes this statement hold.  

For all $r>0$, pick $i_{r}>0$ such that $d\left(a,a_{i_{r},n_{r}}\right)=r$ (note that since $\left\{ a_{i,n_{r}}\right\} _{i\in\mathbb{N}}$ is a path in $\mathcal{G}\left(\Sigma\right)$, we have $i_{r}\geq r$). Then $\left\{ a_{i_{r},n_{r}}\right\} _{r\in\mathbb{N}}$ is an unbounded sequence, which is contained in $N_{C}\left(\left\{ a_{i,0}\right\} _{i\in\mathbb{N}}\right)$, so that $\lim_{r\to\infty}a_{i_{r},n_{r}}=P_{0}$. On the other hand, for any $K\subset\Sigma$ compact and $\epsilon>0$, we can choose $r$ and $n_{r}$ sufficiently large so that $a_{i_{r},n_{r}}\in U_{K,\epsilon/2}\left(\mu_{n_{r}}\right)$ (since $\left\{ a_{j,n_{r}}\right\} _{j\in\mathbb{N}}$ CHCCS-converges to $\mu_{n_{r}}$) and $\mu_{n_{r}}\in U_{K,\epsilon/2}\left(\mu_{0}\right)$ (since $\left\{ \mu_{j}\right\} _{j\in\mathbb{N}}$ CHCCS-converges to $\mu_{0}$). Thus, $a_{i_{r},n_{r}}\in U_{K,\epsilon}\left(\mu_{0}\right)$, and $\left\{ a_{i_{r},n_{r}}\right\} _{r\in\mathbb{N}}$ CHCCS-converges to $\mu_{0}$. Thus, $\Phi\left(\mu_{0}\right)=P_{0}$, by Proposition \ref{prop:bounded_Haus_dist}. 
\end{proof}


\begin{lem} \label{lem:5.3.1}
Suppose $\lambda\in\mathcal{H}\left(\Sigma\right)$, and $m\in\mathbb{N}$. Then for any compact witness $K\subset\Sigma$ and $\epsilon>0$, $\exists R>0$ such that for any $x\in\mathcal{G}\left(\Sigma\right)$ which is disjoint from $\lambda\left(\left[-R,R\right]\right)$, and any $y\in\mathcal{G}\left(\Sigma\right)$ such that $d_{\mathcal{G}}\left(x,y\right)\leq m$, we have $y\in U_{K,\epsilon}\left(\lambda'\right)$ for some $\lambda'$ in the connected component of $\lambda$ in $\tilde{\mathcal{G}}\left(\Sigma\right)$.
\end{lem}

\begin{proof}
Suppose for contradiction, for any $R>0$, there exists $x_{R},y_{R}\in\mathcal{G}\left(\Sigma\right)$ such that 
\begin{enumerate}
\item $d_{\mathcal{G}}\left(x_{R},y_{R}\right)\leq m$.
\item $x_{R}$ is disjoint from $\lambda\left(\left[-R,R\right]\right)$.
\item $y_{R}\notin U_{K,\epsilon}\left(\lambda'\right)$ for any $\lambda'$ in the connected component of $\lambda$ in $\tilde{\mathcal{G}}\left(\Sigma\right)$. 
\end{enumerate}
For each $R$, we can form a path 
\[
x_{R}=x_{R}^{0}-x_{R}^{1}-\dots-x_{R}^{m}=y_{R}
\]
in $\mathcal{G}\left(\Sigma\right)$. By Lemma \ref{lem:CHCCS_seq_cpct}, up to choosing a subsequence, let $\left\{ x_{R}\right\} _{R\in\mathbb{N}}\xrightarrow{\mathrm{CHCCS}}\mu_{0}$, where $\mu\in\mathcal{H}\left(\Sigma\right)$ is disjoint from $\lambda$. Similarly, up to choosing subsequences, each $\left\{ x_{R}^{i}\right\} _{R\in\mathbb{N}}\xrightarrow{\mathrm{CHCCS}}\mu_{i}$. Moreover, by Lemma \ref{lem:disjoint_pts_at_infinity}, we get a path 
\[
\mu_{0}-\mu_{1}-\dots-\mu_{m}
\]
in $\tilde{\mathcal{G}}\left(\Sigma\right)$. 

Now, $\mu_{m}$ is in the connected component of $\lambda$, by construction. On the other hand, a subsequence of $\left\{ y_{R}\right\} _{R\in\mathbb{N}}$ CHCCS-converges to $\mu_{m}$. Thus, for $R$ large enough, we must have $y_{R}\in U_{K,\epsilon}\left(\mu_{m}\right)$, which is a contradiction. 
\end{proof}

\begin{prop} \label{prop:5.3.2}
Let $P\in\partial\mathcal{G}\left(\Sigma\right)$. For every compact witness $K\subset\Sigma$ and $\epsilon>0$, there exists $N$ such that for every quasi-geodesic path $\left(y_{n}\right)_{n\in\mathbb{N}}$ in $Q\in U\left(P,N\right)\subset\partial\mathcal{G}\left(\Sigma\right)$, there exists some $\eta\in\Phi^{-1}(P)$ such that $y_{p}\in U_{K,\epsilon}\left(\eta\right)$ for some $p$. 
\end{prop}

\begin{proof}
Let $P\in\partial\mathcal{G}\left(\Sigma\right)$, and let $\mu\in\mathcal{H}\left(\Sigma\right)$ such that $\Phi\left(\mu\right)=P$ (this follows from the surjectivity of $\Phi$). Let $a\in\mathcal{G}\left(\Sigma\right)$ and $\epsilon>0$ such that $N_{\epsilon}\left(a\right)$ is properly embedded in $\Sigma$ and is homeomorphic to $\mathbb{R}\times\left[-\epsilon,\epsilon\right]$. \textcolor{red}{CITATION - USE THE NIELSEN CONVEX STUFF HERE.}

Note that for any $\lambda\in\mathcal{H}\left(\Sigma\right)$, consecutive points of $a\cap\lambda$ are at least distance $\epsilon$ apart along $\lambda$. So, if $\left\{ x_{n}\right\} \subset\mathcal{B}\left(a,\lambda\right)$ is the bicorn path obtained from Lemma \_\_ by starting at $\lambda(0)$, then $x_{n}$ is disjoint from $\lambda\left(\left[-\frac{n\epsilon}{2},\frac{n\epsilon}{2}\right]\right)$. 

Let $\left(x_{n}\right)\subset\mathcal{B}\left(a,\mu\right)$ be a quasi-geodesic bicorn path CHCCS-converging to $\mu'$ disjoint from $\mu$. Let $\left(y_{n}\right)$ be a quasi-geodesic bicorn path converging to $Q\in\partial\mathcal{G}$. If $Q\in U\left(P,N\right)$, then we have $\liminf_{i,j\to\infty}\left(x_{i},y_{j}\right)_{a}\geq N-2\delta$. Let $N'=N-2\delta$. Choose $i>N'+1$, and $j$ s.t. $\left(x_{i},y_{j}\right)_{a}\geq N'$. Then any two geodesics $\left[a,x_{i}\right]$ and $\left[a,y_{j}\right]$ have their first $N'$ terms $2\delta$-close. 

Let $R>0$ be as in the previous lemma. Choose $N$ large so that $\left(N'+1\right)\frac{\epsilon}{2}>R$. Since bicorn paths are uniform quasi-geodesics, we get that for some $p\in\mathbb{N}$, $y_{p}$ is in a $C$-neighbourhood of $x_{N'+1}$, where $C$ is a constant depending only on $\delta$. By construction, $x_{N'+1}$ is disjoint from $\mu\left(\left[-R,R\right]\right)$, so that $y_{p}\in U_{K,\epsilon}\left(\lambda'\right)$ for some $\lambda'$ in the connected component of $\mu$ in $\tilde{\mathcal{G}}\left(\Sigma\right)$. 
\end{proof}

==> Old_versions/grand_loops.tex <==
%%%% Currently not in use, as not needed. The math here seems correct, and could be useful in future(?)


\section{Grand Loops}

\textcolor{red}{In this section, we define the grand loops graph, and prove that it is quasi-isometric to the grand arc graph.}

\begin{defn}
    Let $\Sigma$ be an infinite-type surface.
    A \textit{loop} in $\Sigma$ is a simple arc with both endpoints converging to the same end.

    A loop $l$ is called \textit{grand} if it satisfies the following conditions:
    \begin{enumerate}
        \item Both endpoints of $l$ are maximal
        \item $l$ is separating
        \item Both connected components of $\Sigma \backslash l$ contain a grand arc.
    \end{enumerate}
\end{defn}

\begin{rmk}
    The third condition above is equivalent to there being  a maximal end in each connected component of $\Sigma\backslash l$.
\end{rmk}

\begin{lem}
    A loop is grand if and only if it is witness filling
\end{lem}

\begin{proof}
    TODO
    \textcolor{red}{ABN: I strongly suspect that this is true. One direction is easy: if the
    loop is grand, and not witness-filling, then there must be a witness
    contained in one connected component of $\Sigma \ssm l$, but then $l$ could
    not contain a grand arc in the other component. 
    }
\end{proof}

\begin{defn}
    The \textit{grand loop graph} $L(\Sigma)$, is the graph whose vertices are
    homotopy classes of grand loops, with edges between loops when they can be
    realized disjointly.
\end{defn}

The rest of this section is dedicated to proving the following lemma:

\begin{lem}
    $\calG(\Sigma)$ and $L(\Sigma)$ are quasi-isometric.
\end{lem}

To prove that these graphs are quasi-isometric, we construct two coarsely-defined Lipschitz maps, 
$f:L(\Sigma) \to \calG(\Sigma)$ and $g:\calG(\Sigma) \to L(\Sigma)$ as follows:
$$
    f(l) = \{\alpha \in \calG(\Sigma): |\alpha\cap l| = 0\}\\
    g(\alpha) = \{l \in L(\Sigma): |l\cap \alpha| = 0\}
$$

\begin{claim}
    $f$ and $g$ are coarsely well-defined. That is, for any $l \in L(\Sigma)$ 
    and $\alpha \in \calG(\Sigma)$, $\mathrm{diam}(f(l))$ 
    and $\mathrm{diam}(g(\alpha))$ are bounded uniformly.
\end{claim}

\begin{proof}
    We start by showing that $\mathrm{diam}(f(l)) \le 3$. Let $\alpha,\beta$ be
    grand arcs disjoint from $l$. If $\alpha$ and $\beta$ lie in distinct
    connect components of $\Sigma \ssm l$, then they must be disjoint. If 
    they lie in the same component, then any grand arc in the other component 
    must be disjoint from both. Thus, $d_{\calG(\Sigma)}(\alpha,\beta) \le 3$.

    Next, we show that $\mathrm{diam}(g(\alpha)
    
    

Claim:
For any $l$, $f(l)$ has diameter at most $2$.

Proof: Let $\Sigma_1,\Sigma_2$ be the connected components of $\Sigma \setminus l$, and let $\alpha,\beta$ be grand arcs disjoint from $l$. Up to replacing $\alpha$ with $\alpha' \in f(l)$ disjoint from $\alpha$, we can assume WLOG that $\alpha,\beta \subset \Sigma_1$. For any grand arc $\gamma \subset \Sigma_2$, we have $\alpha - \gamma -\beta$, and we're done.

Claim:

Suppose that $\Sigma$ has at least four maximal end types.
If $l_1,l_2$ are disjoint grand loops, then $f(l_1)$ and $f(l_2)$ intersect.

Proof: Let $\Sigma_1,\Sigma_2$ be the conn comp. comp. of $l_1$, WLOG $l_2$ is contained in $\Sigma_2$, and separates $\Sigma_3$ from a part of $\Sigma_2$. Any grand arc contained in $\Sigma_3$ will do.

**Notation**
$e(l)$ is the end that $l$ converges to.

Claim:

Suppose that $\Sigma$ has exactly three max end types, then $f(l_1)$ and $f(l_2)$ are close.

If $l_1$ and $l_2$ are disjoint, see above. Suppose $e(l_1)$ and  $e(l_2)$ are in distinct equivalence classes. Let $U(l_1,l_2)$ be the set of all unicorns between $l_1$ and $l_2$. 

Note that $|U(l_1,l_2)| \le 4$, and $U(l_1,l_2)$ consists of grand arcs. This means that there exists a sequence $x_1,...,x_n$ (with $n < 5$) such that $l_1 - x_1 - x_2 - x_3 - .. - x_n - l_2$ where  ( - ) means disjointness. In particular, $x_1 \in f(l_1)$ and $x_n \in f(l_2)$. So these sets are close.

If $e(l_1)$ and $e(l_2)$ are in the same equivalence class then pick maximal $e \in E(\Sigma)$ not equivalent to $e(l_i)$. Pick a path $\gamma$ from $e$ to $l_1$ which does not intersect $l_2$. $\gamma$ intersects $l_1$ at $p$, and the unicorn $x = \gamma *_p l_1$ is a grand arc disjoint from $l_1$, and which intersects $l_2$ at most twice.

Let $q$ be the first intersection of $x$ with $l_2$, since $|x \cap l_2| \le 2$, there exists a direction along $l_2$ for which $x_1 = x *_q l_2$ is simple and disjoint from $l_2$, and intersects $x$ at most once. Now, the standard "sidestep unicorn" argument for grand arcs will work between $x$ and $x_1$, so $d_G(x,x_1) < 4$,

$$
l_1 - x - \cdots - x_1 - l_2
$$

**In fact**:
We can use some combinatorics to show that regardless of the number of maximal ends ($\ge 3$), $f(l_1)$ and $f(l_2)$ intersect. 

Proof idea: 
Look at the intersections of the surfaces that $l_1$ and $l_2$ separate, and find a grand arc between them (uses a very strict constraint on the number of complementary components of $\Sigma \smallsetminus (l_1 \cup l_2))$.

---

**Define**
$g: G \to L$ sending $\alpha \to \{l : |l\cap \alpha| = 0\}$.

Claim:
For any $\alpha$, $g(\alpha)$ has finite diameter.

Proof:

Let $c$ be a simple closed curve int
**Proof missing**


Claim:

If $\alpha \sim \beta$ then $g(\alpha)$ and $g(\beta)$ are close.

Proof:

If there exists an end of $\beta$ which is not an end of $\alpha$, (use FGM + Grand arcs paper) choose $c$ to be a simple closed curve disjoint from $\alpha$, intersecting $\beta$ exactly once, and separating an end of $\beta$ from the rest of the ends of $\alpha$. Then $\beta * c * \beta$ is a grand loop disjoint from both $\alpha$ and $\beta$. 

If $e(\alpha) = e(\beta)$, find $\gamma$ disjoint from $\alpha$ and $\beta$ with different ends, and then $g(\alpha)$ intersects $g(\gamma)$ which intersects $g(\beta)$.




    

